Ternary Neural Networks with Fine-Grained Quantization

We propose a novel fine-grained quantization (FGQ) method to ternarize pre-trained full precision models, while also constraining activations to 8 and 4-bits. Using this method, we demonstrate a minimal loss in classification accuracy on state-of-the-art topologies without additional training. We provide an improved theoretical formulation that forms the basis for a higher quality solution using FGQ. Our method involves ternarizing the original weight tensor in groups of $N$ weights. Using $N=4$, we achieve Top-1 accuracy within $3.7\%$ and $4.2\%$ of the baseline full precision result for Resnet-101 and Resnet-50 respectively, while eliminating $75\%$ of all multiplications. These results enable a full 8/4-bit inference pipeline, with best-reported accuracy using ternary weights on ImageNet dataset, with a potential of $9\times$ improvement in performance. Also, for smaller networks like AlexNet, FGQ achieves state-of-the-art results. We further study the impact of group size on both performance and accuracy. With a group size of $N=64$, we eliminate $\approx99\%$ of the multiplications; however, this introduces a noticeable drop in accuracy, which necessitates fine tuning the parameters at lower precision. We address this by fine-tuning Resnet-50 with 8-bit activations and ternary weights at $N=64$, improving the Top-1 accuracy to within $4\%$ of the full precision result with $<30\%$ additional training overhead. Our final quantized model can run on a full 8-bit compute pipeline using 2-bit weights and has the potential of up to $15\times$ improvement in performance compared to baseline full-precision models.

==> acknowledgment.tex <==
\section*{Acknowledgment}
We thank Prof Bo Zhang and Fengfu Li for providing us the proof of closed-form solution of optimal threshold  of TWN (\cite{2016twn}) under Gaussian assumption.

==> alg_TwoR.tex <==
\begin{algorithm}[t]
\centerline{
\caption{Ternarize Weights}\label{alg:TwoR}
}
\begin{algorithmic}[1]
%--------------------------------------------------
\State \textbf{Input:} Learned full-precision weights $\matW$ of a layer with $d$ filters.
%--------------------------------------------------
%
\State Group filters into $k$ clusters: $\{G_j\}, j=1,..., k$. 
Let $N = \sabs{G_j}$ (number of filters in $G_j$).
\State For each cluster $G_j$
\State \quad Run Algorithm \ref{alg:threshold} on each filter $\matW \in G_j$, and store the thresholds as a vector $\alpha$.% (length $s_j$). 
\State \quad For $t=1,..., N$, \quad 
$T_t=\{i: \alpha_i \text{ belongs to the top } t \text{ elements of sorted } \alpha\}$.
\State \qquad Set $\alpha_t  = \sqrt{\sum_{i\in T_t}\alpha_i^2/\sabs{T_t}}$. 
\State \qquad Construct $\hat\matW{}^{(t)}$, such that, $\hat\matW{}^{(t)}_i = Sign(\matW_i)$, if $\sabs{\matW_i} > \alpha_t$, and 0 otherwise.
\State \quad Find $\alpha_{t^*}$ and $\hat\matW{}^*{}^{(t)}$ that minimizes 
$\sum_{\matW\in G_j}\FsNorm{\matW-\alpha_t\hat\matW{}^{(t)}}^2$.
\State \quad Let $\hat\alpha_{t^*}$ be a reduced-precision representation of $\alpha_{t^*}$.
\State \textbf{Output:} $k$ number of $\hat\alpha_{t^*}$ and the group of ternary weights $\hat\matW$.
%
\end{algorithmic}
\end{algorithm} 


==> alg_threshold.tex <==
\begin{algorithm}[t]
\centerline{
\caption{Threshold Selection}\label{alg:threshold}
}
\begin{algorithmic}[1]
%--------------------------------------------------
\State \textbf{Input:} $\matW \in \mathbb{R}^n$.
%--------------------------------------------------
%
\State Sort elements of $\matW$ according to magnitude.
\State For $\tau \in [0,1]$, $I_\tau=\{i: \sabs{\matW_i} \text{ belongs to the top } \floor{\tau\cdot n} \text{ elements of sorted list}\}$.
\State Construct $\hat\matW{}^{(\tau)}$, such that, $\hat\matW{}^{(\tau)}_i = Sign(\matW_i)$, for $i \in I_\tau$, and 0 otherwise.
\State Set $\alpha_\tau = \sqrt{\sum_{i\in I_\tau} \matW_i ^2/\sabs{I_\tau}}$.
\State Compute $\alpha_{\tau^*}$ that minimizes 
$\FsNorm{\matW-\alpha_\tau\hat\matW{}^{(\tau)}}^2$, for $\tau \in [0,1]$.
\State \textbf{Output:} $\alpha_{\tau^*}$
%
\end{algorithmic}
\end{algorithm} 


==> formulation.tex <==
\section{Dynmaic fixed point - Numerical scheme}

\begin{equation} \label{eq:dfp_1}
\begin{split}
I = \frac{f*2^{N}}{2^{sf}}, \\
sf = Exponent - 127
\end{split}
\end{equation}

==> inference.tex <==
\section{Low Precision Inference}{\label{sec_lpinf}}
In this paper, we primarily focus on improving the performance and accuracy of the inference task. We explore possibility of achieving high accuracy using sub 8-bit precision on state-of-the-art networks without expensive retraining. Previous work from Miyashita et al.\cite{logqunat} showed that by compressing the dynamic range of the input, it is possible to minimize the quantization loss and achieve high accuracy. 
We take a different approach to minimize the impact of dynamic range on quantization. We propose a cluster-based quantization method that groups weights into smaller clusters and quantize each cluster with a unique scaling factor. We use static clustering to group filters that accumulate to the same output feature to simplify the convolution operations. Empirical evidence also suggests that these clusters which learn similar features tend to have smaller dynamic range. Using dynamic fixed point representation, this method can effectively minimize the quantization errors and improve the inference accuracy of quantized networks. Applying this scheme on a pre-trained Resnet-101 model, with $4$-bit weights and $8$-bit activations, we achieve $76.3\%$ TOP-1 accuracy on ImageNet dataset\cite{imagenet_data}, without any retraining.

\subsection{2-bit Ternary Weights}
{\label{sec_ternary}}
Going below 4-bits we use the the ternary representation for weights, following the threshold based approximation proposed by Li et al \cite{2016twn}, i.e., approximate full-precision weight $\matW \approx \alpha\hat\matW$ in $\ell_2$ norm $\FsNorm{\cdot}$, where $\alpha$ is a scaling factor and $\hat\matW$ is a ternary weight with $\hat\matW_i \in \{-1,0,+1\}$. Where $\matW$ is the matrix representing learned full-precision weights, and $\hat\matW$ represents the corresponding ternary representation. We apply the block-quantization method described in section-\ref{sec_lpinf}, to compute multiple scaling factors for each layer to minimize the accuracy loss.  
 %Then, $\matW \approx \matD\hat\matW$, where $\matD$ is a diagonal matrix containing the scaling factors. 
Our method differs from \cite{2016twn} in the approximation used for computing scaling factor ($\alpha$). We use the $RMS$ formulation as shown by the equation (\ref{eq_1}). The intuition behind using $RMS$ term is to push the threshold parameter towards larger values within the cluster which helps speed up weight pruning.

\begin{equation}\label{eq_1}
\alpha = \sqrt[]{\dfrac{{\sum_{i\in I_\tau} \matW_i ^2}}{\abs{I_\tau}}}, \text{where } \abs{I_\tau} \text{ is the number of elements in } I_\tau. 
\end{equation}

In addition, we run our search algorithm\ref{alg:TwoR} in hierarchical fashion by minimizing the error within each filter first and then within the cluster of filters. Experimental evidence shows that these improvements help finding the optimal scaling factor that minimizes quantization loss.

%More specifically, we first use a hierarchical search algorithm \comment{D}{might be good elaborate on the heirarchical search algo - @Naveen ?} to cluster the kernels of a given layer, and then compute a scaling factor for each group of kernels. 
Using multiple scaling factors can lead to more 8-bit multiplications. Hence, we choose the cluster size carefully to improve the ratio of low-precision (2-bit) to high-precision (8-bit) operations (Section \ref{sec_perfimpl}).
%Going below 4-bits we use the ternary representation for weights, following the threshold based approximation proposed by Li et.al.\cite{2016twn}.But our method uses different approximation to compute the scaling factor $\alpha$ as shown in \eqref{eq_1}. In addition, we use clustering mechanism described in \ref{sec_perfimpl} to compute multiple scaling factors for each layer. We use a hierarchical search algorithm described below to compute the scaling factor for each cluster.
Our algorithm (Algorithm \ref{alg:TwoR}) takes the full-precision learned weights and returns clusters of ternary representation of groups of kernels along with their scaling factors. We further quantize the scaling factors down to 8-bit to eliminate any operation that requires more than 8 bits. Applying this scheme on pre-trained ResNet-101 model, using 8-bit activations we achieve $71.8\%$ TOP-1 accuracy on ImageNet dataset.

\input{alg_TwoR}
\input{alg_threshold}

%Going below 4-bits we use the ternary representation for weights, following the threshold based approximation proposed by Li et.al.\cite{2016twn}.Our method differs in the approximation used to compute the scaling factor $\alpha$; nstead of using the mean, we use the RMS value  as shown in \eqref{eq_2}. In addition, we use a hierarchical search algorithm for minimizing the Euclidian norm within the selected group of filters, sweeping from individual filters all the way to full set of weights within that group. Experimental evidence shows that these improvement help minimize the quantization error. 

%\begin{equation}
%\label{eq_1}
%\begin{split}
% =  \sum_{i=0}^{n}\frac{(W_{i}-\alpha\hat{W}_{i})^2}{W_{i}^{2}}, %\quad where \hat{W}_{i} \in {-1,0,1} 
%\end{split}
%\end{equation}
%\begin{equation}
%\label{eq_2}
%\begin{split}
%\alpha = RMS(W_{i}), \quad for \quad ||W_{i}|| < W_{t}
%\end{split}
%\end{equation}

%We further quantize the scaling factor $\alpha$ down to 8-bit making to eliminate all high-precision 32-bit operations. Applying this scheme on pre-trained Resnet-101 model, using $8$-bit activations we achieve $71.8\%$ TOP-1 accuracy on Imagenet dataset. 

\subsection{C1 and BatchNorm Layers} 
In our experiments we keep weights of the first convolution layers at $8$-bits to prevent from accumulating losses while the rest of the layers including fully connected layers operate at lower precision. We also recompute the batch norm parameters during the inference phase to compensate for the shift in variance introduced by quantization. This is essential for making it work, when we are not retraining at lower precision. We are exploring the possibility of fusing batch normalization layers with the convolution layers before quantization to avoid this extra computation. 

\begin{figure}[h]
\centering
\includegraphics{plots/resnet101-notrain.png}
\centering
\caption{Resnet-101 results on ImageNet dataset using 8-bit activations with 4-bit weights $8a-4w$ and 2-bit weights $8a-2w$} \label{fig_res101}
\end{figure}

\subsection{Performance Implications}
{\label{sec_perfimpl}}
Choosing the right cluster size is a trade-off between  performance and accuracy, while having one cluster per layer favors higher compute density by eliminating all multiplications, it's not ideal for achieving high accuracy. Although, previous research in this space\cite{venkatesh2016} showed that it is possible to recover some of this lost accuracy through retraining. It's not always ideal, because of the costs involved in retraining these networks in low-precision, not to mention the technical difficulties involved in achieving reasonable solution on these networks. 

We explored the accuracy-performance trade-off with various cluster sizes. Our experiments show on Resnet-101, using a cluster size of $N=4$ can achieve $71.8\%$ TOP-1 accuracy, within $6\%$ of the full precision result. This result significant because this is to the best of our knowledge highest accuracy achieved on Imagenet dataset\cite{imagenet_data} without retraining the network in low-precision. In terms of performance impact, the clustering will result in one 8-bit multiplication for the entire cluster ($N*K^2$) of ternary accumulations. Assuming roughly $50\%$ of the convolutions are 3x3 and the rest are 1x1, using this block size can potentially replace $85\%$ of multiplications in Resnet-101 convolution layers with simple $8$-bit accumulations. For networks that predominantly use filters that are 3x3 or bigger, this ratio would be greater than $95\%$. We explored the accuracy-performance trade-off with various cluster sizes, we concluded that using cluster size of $N=64$, we can replace $\approx98\%$ of multiplications in Resnet-101 with $8$-bit accumulations, but with a significant loss to the accuracy. At this point retraining the network at lower precision would be necessary.

%In addition we use a hierarchical search algorithm for minimizing the Euclidean norm \eqref{eq_1}, sweeping across the filters. This method is more effective in minimizing the quantization error which leads to better accuracy when we are not retraining. Using this method we group the weights along the output dimension and assign a scaling factor $(\alpha)$ for each group. We have chosen the group size to minimize the number of multiplication at each layer.  Further, we quantize the scaling factors to 8b in order to keep all computation in the convolution layers in 8b. All our fixed point operations use  32b for accumulator to minimize the overflow errors. The 32b output is then clipped and stochastically rounded to an 8b fixed point value.%


==> new_formulation_main_backup.tex <==
\section{Ternary Conversion of Trained Network}{\label{sec_ternaryconversion}}
Our goal is to convert the full-precision trained weights $\matW$ to ternary values $\{-\alpha, 0, +\alpha\}$, $\alpha\geq 0$, without re-training. We use a threshold ($\Delta>0$) based approach similar to \cite{2016twn}: $i$-th element $\hat\matW_i = sign(\matW_i)$, if $\sabs{\matW_i}> \Delta$, and $0$ otherwise.
Then, the element-wise error is  $E(\alpha,\Delta)=\FsNorm{\matW-\alpha\hat\matW}^2$ and an optimal ternary representation $\alpha^*\hat\matW{}^*\approx \matW$ is as follows: 
\begin{eqnarray}\label{eqn:twn}
%\alpha^*, \hat\matW{}^* &=& \argmin_{\alpha,\hat\matW}\FsNorm{\matW-\alpha\hat\matW}^2, \\
\alpha^*, \Delta^* &=& \argmin_{\alpha\geq 0,\Delta>0}E(\alpha,\Delta) 
%= \argmin_{\alpha\geq 0,\Delta>0}
%\FsNorm{\matW-\alpha\hat\matW}^2
\\
\text{ s.t. }
\nonumber 
&& \alpha \ge 0, \hat\matW_i\in \{-1,0,+1\}, i=1,2,...,n
\end{eqnarray} 
where $n$ is the size of $\matW$ ($\matW \in \mathbb{R}^n$).
%However, we have noticed that this formulation gives us poor approximation when we ternarize weights without retraining. 
%
%The reason could be the following. 
%We have the following observations:
%\\
We hypothesize that weights that learn different types of features 
%, i.e., weights of different filter 
may follow different distributions. Combining all the weights together represents a mixture of various distributions, 
%with different parameters (controlling different dynamic range), 
and  ternarizing them using a single threshold ($\Delta$) and magnitude ($\alpha$) may not preserve the distributions of individual weights. Consequently, many weights are approximated poorly (if not totally pruned out) leading to lose of valuable information that they learn. We may not be able to compensate for this loss of information as we do not train the network in low precision. 

%recalibrate weights using re-training. 
%This problem demands a more fine-grained approach to ternarization that  minimizes the loss of accuracy due to quantization. %is suitable for our current scenario.
%One way to achieve this is to split the problem into independent subproblems, 
%and ternarize them separately. For each sub-problem, 
%
Further refinement of this solution maybe possible 
as we hypothesize that positive and negative weight distributions are not always symmetric to each other. In such cases, we intend to use two separate thresholds $\Delta_p, \Delta_n >0$, along with separate scaling factors $\alpha_p, \alpha_n \geq 0$,  
%and one $\alpha$ 
to ternarize the positive and negative weights independently. 

We can consider the weights as a vector $\matW$, and we can decompose $\matW$ into two orthogonal component vectors $\matW_p$ and $\matW_n$ containing positive and negative values, respectively, such that $\matW = \matW_p + \matW_n$. We can find the ternary representation for these components separately: $\hat\matW_{p_i}=1$, if $\matW_{p_i}>\Delta_p$, and 0 otherwise. Similarly, $\hat\matW_{n_i}=-1$, if $\matW_{n_i}<-\Delta_n$, and 0 otherwise. Then we have the following optimal ternary sub-problems.
\begin{eqnarray*}
\alpha_p^*,\Delta_p^* &=& \argmin_{\alpha_p\geq0, \Delta_p>0}\FsNorm{\matW_p - \alpha_p\hat\matW_p}^2
\\
\alpha_n^*,\Delta_n^* &=& \argmin_{\alpha_n\geq0, \Delta_n>0}\FsNorm{\matW_n - \alpha_n\hat\matW_n}^2
\end{eqnarray*}
The usage of two separate scaling factors increases the model capacity, as argued by \cite{zhu2016ttq}.  
However, separate scaling factors $\alpha_p^*$ and $\alpha_n^*$, despite improving the accuracy, typically makes the inference computationally inefficient by necessitating multiple passes over positive and negative values, increasing the bandwidth requirements.

\subsection{Our Formulation}{\label{sec_formulation}}
Computing separate $\Delta$ and $\alpha$ for each weight compensates for information loss and better preserves the underlying distributions. However, such fine-grained ternarization, despite showing significant improvement in accuracy, typically involves a larger number of multiplications leading to a less efficient implementation. Therefore, we seek to find a trade-off between higher accuracy and lower number of high-precision multiplications. Thus, we propose a fine-grained quantization approach that creates groups of weights, and ternarizes each group independently.  
%
Let us consider the weights represented as a vector $\matW \in \mathbb{R}^n$. We partition the set $I$ of $n$ indices into $k$ disjoint subsets, $c_1, c_2, ..., c_k$, with cardinality $\sabs{c_i}=n_i$, such that, $c_i\cap c_j = \emptyset$, $\cup_i c_i = I$, $\sum_in_i = n$. We can decompose $\matW$ into $k$ orthogonal vectors $\matW^{(i)} \in \mathbb{R}^n$, $i=1,...,k$, where $j$-th component $\matW^{(i)}_j=\matW_j$ if $j \in c_i$, otherwise $0$. Clearly, $\sum_i \matW^{(i)} = \matW$; then we ternarize each orthogonal component $\matW^{(i)}$ as $\alpha_i\hat\matW{}^{(i)}$, where components of $\hat\matW{}^{(i)}$ are in $\{-1, 0, +1\}$. Threshold-based approach never turns $0$ to non-zero, and the following orthogonality holds.
\begin{eqnarray}\label{eqn:orthogonality}
%\left<\matW^{(i)},\matW^{(j)}\right>=0, 
%\left<\hat\matW{}^{(i)},\hat\matW{}^{(j)}\right>=0, 
%\left<\matW^{(i)},\hat\matW{}^{(j)}\right>=0, \text{ for } i\neq j.
\matW^{(i)}\perp\matW^{(j)}, 
\hat\matW{}^{(i)}\perp \hat\matW{}^{(j)}, 
\matW^{(i)}\perp\hat\matW{}^{(j)}, \text{ for } i\neq j
\end{eqnarray}
It follows that,  
$
%\left<\matW^{(i)}-\alpha_i\hat\matW{}^{(i)}, \matW^{(j)}-\alpha_j\hat\matW{}^{(j)}\right>
%= 0, \text{ for } i \neq j.
(\matW^{(i)}-\alpha_i\hat\matW{}^{(i)})\perp (\matW^{(j)}-\alpha_j\hat\matW{}^{(j)})
$, for $i\neq j$.
Then we have
$$
\FsNorm{\matW - \sum_i\alpha_i\hat\matW{}^{(i)}}^2
= 
\sum_i \FsNorm{\matW^{(i)}-\alpha_i\hat\matW{}^{(i)}}^2
$$
This leads to the following optimization. For a given group of $k$  filters $\{\matW^{(i)}\}, i=1,...,k$,
\begin{eqnarray}\label{eqn:main}
\nonumber
&&
\alpha_1^*,...,\alpha_k^*,\hat\matW{}^{(1)}{}^*,...,\hat\matW{}^{(k)}{}^* 
\\
\nonumber
&=& \argmin_{\alpha_i,\hat\matW{}^{(i)}, i=1,...,k}
\FsNorm{\matW - \sum_i\alpha_i\hat\matW{}^{(i)}}^2,
\\
\nonumber
&&s.t., \matW^{(i)}_j\in \{-1,0,+1\}, \forall j
\\
&=&
\sum_i
\argmin_{\alpha_i,\hat\matW{}^{(i)}}
\FsNorm{\matW^{(i)}-\alpha_i\hat\matW{}^{(i)}}^2
\\
\nonumber
&&s.t., \matW^{(i)}_j\in \{-1,0,+1\}, \forall j
\end{eqnarray}
Therefore, we need to solve $k$ independent sub-problems. Note that the solutions to sub-problems are thread-parallel and easily parallelizeable. This formulation allows a better ternary approximation to the original full-precision weights, ensuring that they remain within a neighborhood of the original solution in the complex search space of parameters, despite no re-training. Consequently, we expect the full-precision solution and the ternary counterpart to generalize in a  similar manner.

We can solve each sub-problem using the following approach.  Let $I_\Delta=\{i : \sabs{\matW_i}>\Delta\}$. Then, from (\ref{eqn:twn}),
\begin{eqnarray*}
%\alpha^*, \Delta^* = \argmin_{\alpha\geq 0,\Delta>0}E(\alpha,\Delta) &=& \argmin_{\alpha\geq 0,\Delta>0}
%\FsNorm{\matW-\alpha\hat\matW}^2
%\\
%\frac{\partial}{\partial \alpha} = 0 \Rightarrow 
\alpha^* &=& \left<\matW,\hat\matW\right>/\FsNorm{\hat\matW}^2
= (\sum_{i\in I_\Delta}\sabs{\matW_i})/\sabs{I_\Delta}
\\
\Delta^* &=& \argmax_{\Delta>0}(\sum_{i\in I_\Delta}\sabs{\matW_i})^2/\sabs{I_\Delta}
\end{eqnarray*}
where $\left<\cdot,\cdot\right>$ denotes the inner product. 
To avoid a time-consuming brute force solution \cite{2016twn} showed that $\Delta^* \approx 0.6\sigma \approx 0.7\cdot\sum_i\sabs{\matW_i}/n$, assuming that the weights follow Gaussian distribution with mean 0 and standard deviation $\sigma$. 
%
However, we hypothesize that for  
full-precision learned weights 
%do not necessarily follow Gaussian or uniform distribution. Instead, it seems 
%of some layers, 
exponential or heavy-tailed distributions (e.g. power law) or even a mixture of distributions could better model the probability of magnitude of the weights. Assuming that the magnitude of the learned weights follow exponential distribution with parameter $\lambda$, we  analytically derive the optimal $\Delta^*$ from the following lemma.
%
\begin{lemma}\label{lemma:main}
Using the above notations, 
if $\sabs{\matW_i} \sim exp(\lambda)$, then 
$$
\Delta^* = \argmax_{\Delta>0}(\sum_{i\in I_\Delta}\sabs{\matW_i})^2/\sabs{I_\Delta}
\approx \frac{1}{\lambda} = \sum_i\sabs{\matW_i}/n
$$
\end{lemma}
From this analysis, we see that we need a higher threshold value to prune larger number of smaller elements. This is intuitive from the shape of the model distributions. 
In reality, however, it may not be appropriate to use a single distribution to model the weights of all the layers of a neural network. We can apply Kolmogorov-Smirnov (K-S) test as a goodness-of-fit measure to identify an appropriate reference distribution (here we choose  between Gaussian and exponential), and find  $\Delta^*$ accordingly. We approximate a heavy-tailed distribution by an exponential one by pruning out some of the smaller elements. This gives us an exponential approximation with smaller $\lambda$. Further, we can use maximum likelihood functions to estimate the parameters of such distributions. For Gaussian $\mathcal{N}(0,\sigma)$, estimated $\hat\sigma = \sqrt{\sum_{i=1}^n\sabs{\matW_i}^2/n}=rms(\matW)$, and for exponential case, estimated parameter $\hat\lambda = \sum_{i=1}^n\sabs{\matW_i}/n$.
Based on such refined analysis, we observe significant improvement in the theoretical ternary error over Gaussian assumption of \cite{2016twn} (Figure \ref{fig:err_improvement}). It is interesting to observe that for earlier convolution layers of ResNet-101 trained on ImageNet, the magnitude of the weights follow exponential distribution, whereas for later stages weights are Gaussian. 

\begin{figure}[t]
\centering
\includegraphics[width=.7\columnwidth]{plots/Gaussian_improvement_BN.pdf}
\centering
\caption{Layer-wise improvement of theoretical ternary error (one $\alpha$ per layer) over Gaussian assumption by choosing an appropriate distribution using K-S test for ResNet-101 on Imagenet dataset.} \label{fig:err_improvement}
\vskip -0.2in
\end{figure}

%============================
In the next section, we discuss a strategy to group the weights. % that can be efficiently implemented on general purpose hardware using vector instruction set.
%Recall that multiple $\alpha$ adds to the number of high-precision multiplication. Keeping this in mind we discuss 
\subsection{Weight Grouping }{\label{sec_groupingofweights}}
%\rcomment{NM}{@Abhisek: Add a recap of the discussion about solving sub-problems and few lines about alternate grouping mechanisms}
\begin{figure}[h]
\begin{center}
\centerline{\includegraphics[width=0.7\columnwidth]{plots/clustering_walpha.eps}}
\caption{Static Grouping: $(R\times S)$ sub-groups of $n$ elements from contiguous filters along $C$ dimension, $\alpha_k$ consists of scaling factors.}
\label{fig:clusterdiagrm}
\end{center}
\vskip -0.2in
\end{figure} 

Our formulation (\ref{eqn:main}) assumes a mechanism that groups full-precision weights to ternarize. It is natural to use grouping as an optimization variable to further reduce the error. However, dynamic clustering methods such as $k$-means, despite leading to better accuracy, are not friendly to efficient implementation. For example, solutions that use arbitrarily grouped filters would have to perform partial output accumulations by gathering all the weights that use a common $\alpha$ to achieve reasonable computational efficiency. Our goal is to find a solution that would achieve higher efficiency on general purpose hardware by minimizing the number of multiplications while also attaining higher accuracy. 

Based on empirical evidence, we conclude that partitioning weights along input channels $C$ achieves better results. We further observed that  individual elements at the same location from multiple filters along $C$, have less variance because they learn similar features. Since the elements along $C$ accumulate to the same output feature, this layout is also amenable to vectorization along $K$. Hence, for the purpose of evaluating our theory, we use static groups of weights from contiguous weights along the $C$ dimension. Figure \ref{fig:clusterdiagrm} shows an example of our grouping scheme using $3\times 3$ filters. Using this scheme, for each group of $3\times 3$ ternary filters, there will be a $3\times 3$ filter containing scaling factor ($\alpha$) for each element in the filter, which translates to $N$ ternary operations for one multiplication.

% ==== further refinement ===
\iffalse%==== begin remove ====
%\subsection{Further Fine-tuning}
For each sub-problem, further refinement might be possible as we hypothesize that positive and negative weight distributions are not always symmetric to each other. In such cases, we intend to use two separate thresholds $\Delta_p, \Delta_n >0$, along with separate scaling factors $\alpha_p, \alpha_n \geq 0$,  
%and one $\alpha$ 
to ternarize the positive and negative weights independently. 
We can consider the weights as a vector $\matW$, and, as discussed earlier, we can decompose $\matW$ into two orthogonal component vectors $\matW_p$ and $\matW_n$ containing positive and negative values, respectively, such that $\matW = \matW_p + \matW_n$. We can find the ternary representation for these components separately: $\hat\matW_{p_i}=1$, if $\matW_{p_i}>\Delta_p$, and 0 otherwise. Similarly, $\hat\matW_{n_i}=-1$, if $\matW_{n_i}<-\Delta_n$, and 0 otherwise. Then we have the following optimal ternary sub-problems.
\begin{eqnarray*}
\alpha_p^*,\Delta_p^* &=& \argmin_{\alpha_p\geq0, \Delta_p>0}\FsNorm{\matW_p - \alpha_p\hat\matW_p}^2
\\
\alpha_n^*,\Delta_n^* &=& \argmin_{\alpha_n\geq0, \Delta_n>0}\FsNorm{\matW_n - \alpha_n\hat\matW_n}^2
\end{eqnarray*}
where respective optimal ternary errors are
$$
\epsilon_p^* = \FsNorm{\matW_p - \alpha_p^*\hat\matW_p^*}^2, \quad 
\epsilon_n^* = \FsNorm{\matW_n - \alpha_n^*\hat\matW_n^*}^2.
$$
The usage of two separate scaling factors increases the model capacity, as argued by \cite{zhu2016ttq}.  
However, separate scaling factors $\alpha_p^*$ and $\alpha_n^*$, despite improving the accuracy, typically makes the inference inefficient by increasing the number of high-precision multiplications. This restricts us to have only one scaling factor $\alpha$, along with two thresholds $\Delta_p$ and $\Delta_n$. For this, we suggest the following ternarization.
%
\begin{eqnarray*}
\hat\matW_i = 
\begin{cases} +1, & \text{ if } \quad \matW_i > \Delta_p,
\\
-1, & \text{ if } \quad \matW_i < -\Delta_n,
\\
0, & \text{ otherwise } 
\end{cases}
\end{eqnarray*}
Then, 
we want to find optimal $\alpha^*$, $\Delta_p^*$, and $\Delta_n^*$ by minimizing the error $E(\alpha,\Delta_p,\Delta_n) = \FsNorm{\matW - \alpha\hat\matW}^2$ as:
\begin{eqnarray}\label{eqn:merge_alpha}
\alpha^*,\Delta_p^*,\Delta_n^*
= \argmin_{\alpha\geq 0,\Delta_p>0,\Delta_n>0}
\FsNorm{\matW - \alpha\hat\matW}^2
\end{eqnarray}
Let 
$
I_\Delta^+ = \{i: \matW_i > \Delta_p\}
$, and 
$
I_\Delta^- = \{i: \matW_i < -\Delta_n\}
$. We can write 
\begin{eqnarray*}
E(\alpha,\Delta_p,\Delta_n) 
&=&
\sum_i \matW_i^2 + \alpha^2(\sabs{I_\Delta^+} + \sabs{I_\Delta^-})  
\\
&&- 2\alpha(\sum_{i\in I_\Delta^+}\sabs{\matW_i}+\sum_{i\in I_\Delta^-}\sabs{\matW_i}) 
\end{eqnarray*}
For fixed $\Delta_p$ and $\Delta_n$, $E(\alpha,\Delta_p,\Delta_n)$ attains maxima at 
$$
\alpha^* = \frac{\sum_{i\in I_\Delta^+}\sabs{\matW_i}+\sum_{i\in I_\Delta^-}\sabs{\matW_i}}{\sabs{I_\Delta^+} + \sabs{I_\Delta^-}}
$$
Using this optimal expression we have 
\begin{eqnarray*}
E(\alpha^*,\Delta_p,\Delta_n)
= c - \frac{(\sum_{i\in I_\Delta^+}\sabs{\matW_i}+\sum_{i\in I_\Delta^-}\sabs{\matW_i})^2}{\sabs{I_\Delta^+} + \sabs{I_\Delta^-}}
\end{eqnarray*}
where $c=\sum_i\matW_i^2$. Then, optimal thresholds are 
\begin{eqnarray*}
%\\
\Delta_p^*,\Delta_n^* &=& \argmax_{\Delta_p>0,\Delta_n>0} \frac{(\sum_{i\in I_\Delta^+}\sabs{\matW_i}+\sum_{i\in I_\Delta^-}\sabs{\matW_i})^2}{\sabs{I_\Delta^+} + \sabs{I_\Delta^-}}
\end{eqnarray*}
Note that, for symmetric case $\Delta_p=\Delta_n=\Delta$, this is identical to (\ref{eqn:twn}). It would be interesting to solve this for a mixture of distributions. 
%We leave it as a future work. 
%
%\iffalse % ====== remove =====
Here, we propose an approximation to this problem assuming we can optimize the positive and negative parts separately. Basically, the problem boils down to merging two scaling factors to one. We can merge them as follows. Let $\x=\alpha_p^*\hat\matW_p{}^*+\alpha_n^*\hat\matW_n{}^*$. We form a ternary vector $\hat\matW$, such that, $\hat\matW_i=sign(\x_i)$, if $\sabs{\x_i}>\Delta$, and 0 otherwise. Then, an optimal ternary representation $\alpha^*\hat\matW{}^*$ is
\begin{eqnarray}\label{eqn:merge}
\alpha^*,\Delta^* = \argmin_{\alpha\geq0,\Delta>0}\FsNorm{(\alpha_p^*\hat\matW_p{}^*+\alpha_n^*\hat\matW_n{}^*) - \alpha\hat\matW}^2
\end{eqnarray}
We use this solution $\alpha^*\hat\matW{}^*$ as a proxy for the true optima in (\ref{eqn:merge_alpha}). Then, we have the following guarantee on approximation quality with respect to optimal error $\epsilon_p^*+\epsilon_n^*$.
$$
\FsNorm{\matW - \alpha^*\hat\matW{}^*}^2 - (\epsilon_p^* + \epsilon_n^*) \leq  \FsNorm{(\alpha_p^*\hat\matW_p{}^*+\alpha_n^*\hat\matW_n{}^*) - \alpha^*\hat\matW{}^*}^2
$$
Note that, elements of vector $\x$ (used in (\ref{eqn:merge})) has three unique magnitudes: $0$, $\alpha_p^*$, and $\alpha_n^*$, and we have only $n_p+n_n$ number of non-zero elements, where $n_p$ and $n_n$ denote number of non-zeros in $\hat\matW_p{}^*$ and $\hat\matW_n{}^*$, respectively. Although We can make assumptions about the distribution to solve the ternarization problem, a brute-force method for  (\ref{eqn:merge}) might be acceptable.

%\iffalse%==== begin remove ====
So far we consider ternary representation by minimizing element-wise error between full-precision weights and ternary values. However, it might be possible to improve the ternary representation by preserving the output feature maps produced by the full-precision weights and the ternary weights when applied on data. For a group of filters we want to solve the following.
%
\begin{eqnarray*}\label{eqn:twn_data}
\alpha^*, \hat\matW{}^* &=& \argmin_{\alpha,\hat\matW}\sum_{\x\in\mathcal{X}}\FsNorm{\x\otimes\matW-(\alpha\x)\odot\hat\matW}^2,
%\alpha^*, \Delta^* &=& \argmin_{\alpha\geq 0,\Delta>0}E(\alpha,\Delta) 
%= \argmin_{\alpha\geq 0,\Delta>0}
%\FsNorm{\matW-\alpha\hat\matW}^2
\\
\text{ s.t. }
\nonumber 
&& \alpha \ge 0, \hat\matW_i\in \{-1,0,+1\}, i=1,2,...,n
\end{eqnarray*} 
where $\otimes$ and $\odot$ denote convolution with and without multiplication, respectively, and $\mathcal{X}$ represents the set of input feature map. Note that, the above is a local optimization problem involving a group of filters, and there is no back propagation involved to fine-tune the ternary values.
\fi
% ===== end of remove ====
%
\iffalse % == begin remove ==
\section{Notes}
1. Weights do not necessarily follow Gaussian or uniform distribution. In fact, it turns out that exponential or heavy-tailed distributions could better model the distribution of magnitude of the  weights.
\\
\\
2. Various filters learn different types of features, i.e., different weights may follow different distributions. Applying threshold based ternary representation considering all the weights of a layer together might be a poor approximation, especially when we do not re-train. This is because all the weights together behave like a mixture of various distributions with different parameters (controlling the dynamic range), and  ternarizing them using a single $\Delta$ and $\alpha$ may not preserve the component distributions of individual filters. Consequently, many filters are approximated poorly (if not totally filtered out) and we lose valuable information learned by those filters. 
\\
\\
3. We propose to use multiple $\alpha$s and $\Delta$s to approximate the mixture of distributions more appropriately, say, one $\alpha$ per filter. 
\\
?? SHOW FORMULATION
\\
However, note that very large number of $\alpha$'s, despite showing considerably higher accuracy, may lead to more high-precision multiplication, making inferencing inefficient. 
\\
\\
4. To deal with this problem, we first group the filters, and then find a ternary representation for each such group. 
\\
\\
5. What does this mean in parameter space??
\\
- By minimizing Euclidean distance of FP weights and their ternary counterparts at such fine-grained levels, our ternary solution essentially stay in a close neighborhood of FP solutions in the optimization parameter space, such that, the two solutions generalize in a similar manner. 
\\
\\

%================
\section{New Formulation}
%================
Let $\matM \in \mathbb{R}^{d\times r \times c}$ denote the full precision learned weight tensor for a given layer, where $d$ is the number of convolution filters and each filter is of dimension $r \times c$. We can unroll $\matM$ into a matrix $\matW \in \mathbb{R}^{d \times r\cdot c}$, where each row contains vector representation of a  convolution filter. We intend to find a ternary representation of $\matW$, denoted by $\hat\matW$, such that each element $\hat\matW_i \in \{-1,0,+1\}$. Current literature (reference 5) suggests to solve the following optimization problem in (\ref{eqn:current}).
%
\begin{eqnarray}\label{eqn:current}
\alpha^*, \hat\matW{}^* &=& \argmin_{\alpha,\hat\matW}\FsNorm{\matW-\alpha\hat\matW}^2\\
\nonumber 
&& s.t. \quad \alpha \ge 0, \hat\matW_i\in \{-1,0,+1\}, i=1,2,...,n
\end{eqnarray}
Note that here we approximate the ternary representation using only one scaling factor $\alpha$. However, we found this formulation to be ineffective for conversion of full-precision trained weights to low-precision, when we do not use re-training. Instead, we seek to find an $\alpha$ for each filter (or a sub-group of filters) for better accuracy. Specifically, we intend to solve ()


\subsection{Element-wise $\alpha$}
\begin{eqnarray*}
\matA^*, \hat\matW{}^* &=& \argmin_{\matA,\hat\matW}\FsNorm{\matW-\matA\odot\hat\matW}^2\\
&& s.t. \quad \matA_i \ge 0, \hat\matW_i\in \{-1,0,+1\}, i=1,2,...,n
\end{eqnarray*}

\subsection{Filter-wise $\alpha$}
\begin{eqnarray*}
a_j^*, \hat\matW{}^* &=& \argmin_{a_j,\hat\matW}\sum_j\FsNorm{\matW^{(j)}-a_j\hat\matW{}^{(j)}}^2\\
&& s.t. \quad a_j \ge 0, \hat\matW_i{}^{(j)}\in \{-1,0,+1\}, i=1,2,...,n; j=1,...,d
\end{eqnarray*}
Equivalently, for a diagonal matrix $\matD \ge 0$,
\begin{eqnarray*}
\matD^*, \hat\matW{}^* &=& \argmin_{\matD,\hat\matW}\FsNorm{\matW-\matD\hat\matW}^2\\
&& s.t. \quad \matD_i \ge 0, \hat\matW_i\in \{-1,0,+1\}, i=1,2,...,n;
\end{eqnarray*}
Equivalently, for a diagonal matrix $\matD \ge 0$,
\begin{eqnarray*}
\matW &=& Sign(\matW)\odot\sabs{\matW}
\\
\matD\hat\matW &=& \matD (Sign(\matW)\odot \tilde\matW) 
=  Sign(\matW)\odot (\matD\tilde\matW)
\end{eqnarray*}
\begin{eqnarray*}
\FsNorm{\matW - \matD\hat\matW}^2 &=& \FsNorm{Sign(\matW)\odot\sabs{\matW}
- Sign(\matW)\odot (\matD\tilde\matW)}^2
%\matD\hat\matW &=& \matD (Sign(\matW)\odot \tilde\matW) 
%=  Sign(\matW)\odot (\matD\tilde\matW)
\\
&=& \FsNorm{\sabs{\matW}
- \matD\tilde\matW}^2
\end{eqnarray*}
\begin{eqnarray*}
%\matD^*, \tilde\matW{}^* &=& \argmin_{\matD,\tilde\matW}\frac{\FsNorm{\sabs{\matW}-\matD\tilde\matW}^2}{\FsNorm{\matW}^2}\\
\matD^*, \tilde\matW{}^* &=& \argmin_{\matD,\tilde\matW}\FsNorm{\sabs{\matW}-\matD\tilde\matW}^2\\&& s.t. \quad \matD_i \ge 0, \tilde\matW_i\in \{0, 1\}, i=1,2,...,n;
\\
\hat\matW &=& Sign(\matW)\odot \tilde\matW
\end{eqnarray*}
Optimal $\matD_i^*$ can be computed as, for a given $\hat\w$ (depends on $\Delta^*$,
$$
\matD_i^* = \frac{\w^T\hat\w}{\FsNorm{\hat\w}^2}
$$
$$
\Delta^* = \argmax_{\Delta>0}\frac{1}{\sabs{I_\Delta}}(\sum_{i\in I_\Delta}\sabs{\matW_i})^2
$$
\subsection{Group-wise $\alpha$}

Let diagonal matrix $\tilde\matD$ denote the sub-group of scaling factors, where scaling factors are assigned their cluster centroids. For $k$ sub-groups we have $k$ unique values of  $\tilde\matD$. Also, let $\hat\matD$ denote the low-precision representation of cluster centroids. Then, sub-8 decomposition looks like $\hat\matD\hat\matW$ and the following holds
\begin{eqnarray*}
\FsNorm{\matW-\hat\matD\hat\matW{}^*}
&\leq& 
\FsNorm{\matW-\tilde\matD\hat\matW{}^*}+\FsNorm{\tilde\matD\hat\matW-\hat\matD\hat\matW{}^*}\\
&\leq&
\FsNorm{\matW-\matD{}^*\hat\matW{}^*}+\FsNorm{\matD{}^*\hat\matW{}^*-\tilde\matD\hat\matW{}^*}+\FsNorm{\tilde\matD\hat\matW{}^*-\hat\matD\hat\matW{}^*}\\
&\leq&
\underbrace{\FsNorm{\matW-\matD{}^*\hat\matW{}^*}}_{\text{Ternarization error}}+\underbrace{\FsNorm{\matD{}^*-\tilde\matD}\FsNorm{\hat\matW{}^*}}_{\text{Clustering error}}+\underbrace{\FsNorm{\tilde\matD-\hat\matD}\FsNorm{\hat\matW{}^*}}_{\text{Error for low-precision scaling factors}}\\
\end{eqnarray*}
Error bound due to grouping $\FsNorm{\matD-\tilde\matD}\FsNorm{\hat\matW}$ holds for any grouping (static or dynamic); however, static clustering may give us bigger error whereas optimal clustering $k$-means can make the error smaller. On the other hand, static clustering can give a performance boost while $k$-means may not.

\subsection{Layer-wise $\alpha$}
\begin{eqnarray*}
\alpha^*, \hat\matW{}^* &=& \argmin_{\alpha,\hat\matW}\FsNorm{\matW-\alpha\hat\matW}^2\\
&& s.t. \quad \alpha \ge 0, \hat\matW_i\in \{-1,0,+1\}, i=1,2,...,n
\end{eqnarray*}

%\section{Algorithm: Ternarize-WithOut-Retraining (TwoR)}


%\input{algo_LP}
\subsection{General Bound/Analysis}
$$
E(\hat\w,\alpha) = \FsNorm{\w - \alpha\hat\w}^2
= \FsNorm{\w}^2 - 2\alpha \w^T\hat\w + \alpha^2\FsNorm{\hat\w}^2
$$
Given $\hat\w$, optimal $\alpha^*$ is
$$
\alpha^* = \frac{\w^T\hat\w}{\FsNorm{\hat\w}^2}
$$
$$
E(\hat\w,\alpha^*) 
= \FsNorm{\w}^2 - 2\frac{(\w^T\hat\w)^2}{\FsNorm{\hat\w}^2} + \frac{(\w^T\hat\w)^2}{\FsNorm{\hat\w}^2}
= \FsNorm{\w}^2 - \frac{(\w^T\hat\w)^2}{\FsNorm{\hat\w}^2}
$$
So, minimizing $E$ is maximizing $\frac{(\w^T\hat\w)^2}{\FsNorm{\hat\w}^2}$.
\subsubsection{Ternary Weights}
For ternary representation (keeping weights above some threshold along with their sign)
$$
\w^T\hat\w = \sum_{i\in I_\Delta} \sabs{\w_i}
$$
and
$$
\FsNorm{\hat\w}^2 = \sabs{I_\Delta}
$$

\subsubsection{Binary Weights}
$$
\FsNorm{\hat\w}^2 = n
$$
We want to maximize $\sabs{\w^T\hat\w}$.

\subsection{Quantization using Data}
\begin{eqnarray*}
\matD^*, \hat\matW{}^* &=& \argmin_{\matD,\hat\matW}\sum_{\x\in\mathcal{X}}\FsNorm{\matW\x-\matD\hat\matW\x}^2\\
&& s.t. \quad \matD_i \ge 0, \hat\matW_i\in \{-1,0,+1\}, i=1,2,...,n;
%\end{eqnarray*}
%\begin{eqnarray*}
\\
\alpha_j^*, \hat\matW{}^{(j)}{}^* &=& \argmin_{\alpha_j,\hat\matW}\sum_{\x\in\mathcal{X}}\FsNorm{\matW^{(j)}\x-\alpha_j\hat\matW{}^{(j)}\x}^2\\
&& s.t. \quad \alpha_j \ge 0, \hat\matW_i{}^{(j)}\in \{-1,0,+1\}, i=1,2,...,n; j=1,...,d
\end{eqnarray*}

\section{Residual Precision}
$\matW$ full precision weight\\
$\hat\matW$ ternary weight with 8-bit scaling factor $\hat\alpha$\\
$\Delta = \matW - \hat\alpha\hat\matW$ full precision residual\\
$\hat\Delta$ is ternary residual precision with 8-bit scaling factor $\hat\delta$ 
$$
e = \FsNorm{\matW - (\hat\alpha\hat\matW+\hat\delta\hat\Delta)}
= \FsNorm{\Delta-\hat\delta\hat\Delta}
\geq 
\FsNorm{\Delta}-\FsNorm{\hat\delta\hat\Delta}
$$
$$
\FsNorm{\Delta}-e \leq \FsNorm{\hat\delta\hat\Delta}
$$
Error reduction can be up to $\FsNorm{\hat\delta\hat\Delta}$.

\section{TWN proof}
We want to solve the following
$$
\Delta^* = \argmax_{\Delta>0} \quad \frac{1}{\sabs{I_\Delta}}(\sum_{i\in I_\Delta} \sabs{\matW_i})^2 
$$
\subsection{Uniform case}
Let $\x \sim \mathcal{U}[-a,+a]$. 
%Then, $\mathbb{E}(\sabs{\x}) = \frac{1}{3}a$ as follows.
\begin{eqnarray*}
I(t) = \frac{1}{a}\int_{t}^{a} x dx
= \frac{a^2-t^2}{2a} 
= \frac{(a+t)(a-t)}{2a}
\end{eqnarray*}
$$
\Delta^* = \argmax_t F(t) = \argmax_t \frac{1}{4a^2}\frac{(a+t)^2(a-t)^2}{a-t}
 = \argmax_t \frac{1}{4a^2}(a+t)^2(a-t)
$$
$$
f'(t) = 0 \Rightarrow \Delta^* = a/3
$$
`\subsection{Gaussian case}
Let $\x \sim \mathcal{N}(0,\sigma^2)$. Then, $\mathbb{E}(\sabs{\x}) = 0.8\sigma$ as follows.
\begin{eqnarray*}
I = \frac{1}{\sigma\sqrt{2\pi}}\int_{-\infty}^{\infty}e^{-\frac{\sabs{x}^2}{2\sigma^2}}\sabs{x}dx
= \frac{\sqrt{2}}{\sigma\sqrt{\pi}}\int_{0}^{\infty}e^{-\frac{x^2}{2\sigma^2}}x dx
\end{eqnarray*}
Let $y=\frac{x^2}{2\sigma^2}$, then, $x dx = \sigma^2 dy$
\begin{eqnarray*}
I = {\sigma}\frac{\sqrt{2}}{\sqrt{\pi}}\int_{0}^{\infty} e^{-y}dy
= - {\sigma}\frac{\sqrt{2}}{\sqrt{\pi}} e^{-y}\Big]_0^\infty
= {\sigma}\frac{\sqrt{2}}{\sqrt{\pi}}
\approx 0.8\sigma
\end{eqnarray*}

We want to keep top elements that maximize ratio of the above integral and square root of number of elements we keep.
$$
F(t) = \frac{\sqrt{2}}{\sigma\sqrt{\pi}}\int_{t}^{a}\frac{e^{-\frac{x^2}{2\sigma^2}}x}{\sqrt{a-t}} dx
$$
$$
\argmax_t \quad F(t)
$$
\subsection{Exponential Case}
$$
%\sabs{I_\Delta} = n \int_{x>\Delta} f(x)dx  
\sabs{I_\Delta} \approx n \int_{x>\Delta} f(x)dx 
= n \left(1 - \int_{x <= \Delta} f(x)dx\right)
= n(1-F(\Delta))
$$
where $f(x)=\lambda e^{-\lambda x}$ is pdf of exponential distribution with parameter $\lambda>0$, and $F(x) = 1-e^{-\lambda x}$ is the cdf.
Therefore, 
$$
\sabs{I_\Delta} \approx n e^{-\lambda\Delta}
$$
Furthermore,
$$
\sum_{i\in I_\Delta}\sabs{W_i} \approx n \int_{x>\Delta} x f(x)dx
= n \int_{x>\Delta} (\lambda e^{-\lambda x})x dx
$$
Using integration by parts
$$
\sum_{i\in I_\Delta}\sabs{W_i} \approx n \left(-xe^{-\lambda x}\Big]_{x>\Delta}- \int_{x>\Delta} (-e^{-\lambda x})dx\right)
= n \left(-xe^{-\lambda x}\Big]_{x>\Delta}- \frac{1}{\lambda} e^{-\lambda x}\Big]_{x>\Delta}\right)
$$
From L'hospital's rule
$$
L = \lim_{x \rightarrow \infty}\frac{x}{e^{\lambda x}}
= \lim_{x \rightarrow \infty}\frac{\lambda}{e^{\lambda x}}
= 0
$$
Therefore,
$$
\sum_{i\in I_\Delta}\sabs{W_i} \approx n\left(\Delta e^{-\lambda \Delta}+\frac{1}{\lambda}e^{-\lambda \Delta}\right)
$$
Then,
$$
G(\Delta) = \frac{(\sum_{i\in I\Delta}\sabs{W_i})^2}{\sabs{I_\Delta}}
= \frac{1}{\lambda^2}(1+\lambda\Delta)^2e^{-\lambda\Delta}
$$
$$
G'(\Delta) = \frac{1}{\lambda^2}(2\lambda(1+\lambda\Delta)e^{-\lambda\Delta}-\lambda(1+\lambda\Delta)^2e^{-\lambda\Delta})
$$
$$
G'(\Delta) = 0 \Rightarrow \Delta = \frac{1}{\lambda}
$$
$$
G''(\Delta)\Big|_{\Delta=1/\lambda} < 0 \quad \text{(maxima)}
$$
Therefore,
$$
\Delta^* = \frac{1}{\lambda} = \frac{1}{n}\sum_i\sabs{\matW_i}
$$
\section{Improved Formulation}
\subsection{Two thresholds, two $\alpha$}
Positive and negative values may not be distributed identically. We use separate thresholds and scaling factors for positive and negative weights, and compute respective optima.
\begin{eqnarray*}
I_+ &=& \{i: W_i > \Delta_+\}
\\
I_- &=& \{i: W_i < -\Delta_-\}
\end{eqnarray*}
\begin{eqnarray*}
\Delta_+^* &=& \argmax_{\Delta_+>0} \quad \frac{1}{\sabs{I_+}}(\sum_{i\in I_+} \sabs{\matW_i})^2 
\\
\alpha_+^* &=& \frac{1}{\sabs{I_+}}\sum_{i\in I_+} \sabs{\matW_i}
\\
\Delta_-^* &=& \argmax_{\Delta_->0} \quad \frac{1}{\sabs{I_-}}(\sum_{i\in I_+} \sabs{\matW_i})^2 
\\
\alpha_-^* &=& \frac{1}{\sabs{I_-}}\sum_{i\in I_-} \sabs{\matW_i}
\end{eqnarray*}
We can split $\matW$ into positive and negative components 
$$
\matW = \matW_+ + \matW_-.
$$
Let the corresponding optimal ternary representations be $\alpha_+^*\hat\matW_+^*$ and $\alpha_-^*\hat\matW_-^*$.
\\
The ternarization error is
\begin{eqnarray*}
E &=& \FsNorm{\matW - (\alpha_+^*\hat\matW_+^* + \alpha_-^*\hat\matW_-^* )}^2\\
%\Delta_+^* &=& \argmax_{\Delta_+>0} \quad \frac{1}{\sabs{I_+}}(\sum_{i\in I_+} \sabs{\matW_i})^2 
%\\
%\alpha_+^* &=& \frac{1}{\sabs{I_+}}\sum_{i\in I_+} \sabs{\matW_i}
\end{eqnarray*}

\section{Additional Experiments}

1. Layer-wise $\alpha$: Gaussian TWN vs Exponential vs positive-negative $\alpha$.\\
- plot all the errors
\\
\\
2. Hierarchical vs non-hierarchical\\
- cluster the filters and find one $\alpha$ and $\Delta$ for the entire cluster (without hierarchical )
\\
- 
\section{Bound for Hierarchical}
Split $\w$ into two orthogonal components
$$
\w = \w_p + \w_n
$$
Optimal ternary for $\w_p$ and $\w_n$ are given as $\alpha_p^*\hat\w_p^*$ and $\alpha_n^*\hat\w_n^*$, respectively. 
\begin{eqnarray*}
\epsilon^* 
&=& \FsNorm{\w - \alpha_p^*\hat\w_p^* - \alpha_n^*\hat\w_n^*}^2
= \FsNorm{\w_p - \alpha_p^*\hat\w_p^*}^2 + \FsNorm{\w_n - \alpha_n^*\hat\w_n^*}^2
\end{eqnarray*}
%
\begin{eqnarray*}
\epsilon
&=& \FsNorm{\w - \alpha_p^*\hat\w_p^* - \alpha_n^*\hat\w_n^*}^2
= \FsNorm{\w_p - \alpha_p^*\hat\w_p^*}^2 + \FsNorm{\w_n - \alpha_n^*\hat\w_n^*}^2
\end{eqnarray*}

\section{Mixture Distribution}
Use one $\alpha$ but two thersholds: for positive and negative numbers.
\\
\begin{eqnarray*}
\hat\matW_i &=& 1, \quad if \quad \matW_i > \Delta_p,
\\
\hat\matW_i &=& -1, \quad if \quad \matW_i < -\Delta_n,
\end{eqnarray*}
Let 
$$
I_\Delta^+ = \{i: \matW_i > \Delta_p\}
$$
$$
I_\Delta^- = \{i: \matW_i < -\Delta_n\}
$$
We want to solve
$$
\alpha^*,\Delta_p^*,\Delta_n^*
= \argmin_{\alpha\geq 0,\Delta_p>0,\Delta_n>0}
\FsNorm{\matW - \alpha\hat\matW}^2
$$
\begin{eqnarray*}
E(\alpha,\Delta_p,\Delta_n) &=& \FsNorm{\matW - \alpha\hat\matW}^2
\\
&=&
\sum_i \matW_i^2 - 2\alpha\sum_i\matW_i\hat\matW_i + \alpha^2\sum_i \hat\matW_i{}^2
\\
&=& \sum_i \matW_i^2 - 2\alpha(\sum_{i\in I_\Delta^+}\matW_i\hat\matW_i+\sum_{i\in I_\Delta^-}\matW_i\hat\matW_i) + \alpha^2(\sum_{i\in I_\Delta^+}\hat\matW_i{}^2 + \sum_{i\in I_\Delta^-}\hat\matW_i{}^2)
\end{eqnarray*}
We have
$$
\sum_{i\in I_\Delta^+}\hat\matW_i{}^2
= \sabs{I_\Delta^+},
\quad 
\sum_{i\in I_\Delta^-}\hat\matW_i{}^2
= \sabs{I_\Delta^-}
$$
$$
\sum_{i\in I_\Delta^+}\matW_i\hat\matW_i{}
= \sum_{i\in I_\Delta^+}\sabs{\matW_i},
\quad
\sum_{i\in I_\Delta^-}\matW_i\hat\matW_i{}
= \sum_{i\in I_\Delta^-}\sabs{\matW_i}
$$
$$
\frac{\partial}{\partial\alpha} E(\alpha,\Delta_p,\Delta_n)
= 2\alpha(\sabs{I_\Delta^+} + \sabs{I_\Delta^-}) - 2(\sum_{i\in I_\Delta^+}\sabs{\matW_i}+\sum_{i\in I_\Delta^-}\sabs{\matW_i})
$$
For fixed $\Delta_p$, $\Delta_n$, $E$ attains maxima at 
$$
\alpha^* = \frac{\sum_{i\in I_\Delta^+}\sabs{\matW_i}+\sum_{i\in I_\Delta^-}\sabs{\matW_i}}{\sabs{I_\Delta^+} + \sabs{I_\Delta^-}}
$$
Using this optimal expression we have 
\begin{eqnarray*}
E(\alpha^*,\Delta_p,\Delta_n)
&=& \sum_i\matW_i^2 - \frac{(\sum_{i\in I_\Delta^+}\sabs{\matW_i}+\sum_{i\in I_\Delta^-}\sabs{\matW_i})^2}{\sabs{I_\Delta^+} + \sabs{I_\Delta^-}}
\end{eqnarray*}
\begin{eqnarray*}
\Delta_p^*,\Delta_n^* &=& \argmax_{\Delta_p,\Delta_n} \frac{(\sum_{i\in I_\Delta^+}\sabs{\matW_i}+\sum_{i\in I_\Delta^-}\sabs{\matW_i})^2}{\sabs{I_\Delta^+} + \sabs{I_\Delta^-}}
\end{eqnarray*}
We assume that positive weights follow exponential distribution with parameter $\lambda_1$, and magnitude of negative weights follow exponential distribution with parameter $\lambda_2$.
\\
Let $\gamma\in [0,1]$ be a mixing parameter, i.e., $\gamma n$ number of positive elements and $(1-\gamma)n$ number of negative elements.
$$
\sabs{I_\Delta^+} \approx \gamma n e^{-\lambda_1\Delta_1},
\quad 
\sabs{I_\Delta^-} \approx (1-\gamma) n e^{-\lambda_2\Delta_2}
$$
Furthermore,
$$
\sum_{i\in I_\Delta^+}\sabs{W_i} \approx \frac{\gamma n}{\lambda_1}\left(\lambda_1\Delta_1 + 1\right)e^{-\lambda_1 \Delta_1}
$$
$$
\sum_{i\in I_\Delta^-}\sabs{W_i} \approx \frac{(1-\gamma) n}{\lambda_2}\left(\lambda_2\Delta_2 + 1\right)e^{-\lambda_2 \Delta_2}
$$
\begin{eqnarray*}
E(\alpha^*,\Delta_1,\Delta_2)
&=& 
n\frac{\left(\frac{\gamma}{\lambda_1}\left(\lambda_1\Delta_1 + 1\right)e^{-\lambda_1 \Delta_1} 
+
\frac{1-\gamma} {\lambda_2}\left(\lambda_2\Delta_2 + 1\right)e^{-\lambda_2 \Delta_2}
\right)^2}{\gamma e^{-\lambda_1\Delta_1}+
(1-\gamma) e^{-\lambda_2\Delta_2}}
\end{eqnarray*}
It follows
\begin{eqnarray*}
&&\frac{1}{n}\cdot \frac{\partial}{\partial\Delta_1}E(\alpha^*,\Delta_1,\Delta_2)\\
&=& 
\frac{2\left(\frac{\gamma}{\lambda_1}\left(\lambda_1\Delta_1 + 1\right)e^{-\lambda_1 \Delta_1} 
+
\frac{1-\gamma} {\lambda_2}\left(\lambda_2\Delta_2 + 1\right)e^{-\lambda_2 \Delta_2}
\right)\left[\frac{\gamma}{\lambda_1}(\lambda_1e^{-\lambda_1 \Delta_1}-(\lambda_1\Delta_1+1)\lambda_1e^{-\lambda_1 \Delta_1})\right]}{\gamma e^{-\lambda_1\Delta_1}+
(1-\gamma) e^{-\lambda_2\Delta_2}}
\\
&& -
\frac{\left(\frac{\gamma}{\lambda_1}\left(\lambda_1\Delta_1 + 1\right)e^{-\lambda_1 \Delta_1} 
+
\frac{1-\gamma} {\lambda_2}\left(\lambda_2\Delta_2 + 1\right)e^{-\lambda_2 \Delta_2}
\right)^2}{(\gamma e^{-\lambda_1\Delta_1}+
(1-\gamma) e^{-\lambda_2\Delta_2})^2}\gamma (-\lambda_1) e^{-\lambda_1\Delta_1}
\\
&=&\tau \cdot 
2\left(\gamma e^{-\lambda_1\Delta_1}+
(1-\gamma) e^{-\lambda_2\Delta_2}\right)
\left[\gamma(-\lambda_1\Delta_1)e^{-\lambda_1\Delta_1}\right]
+
\\
&&
\tau \cdot 
\left(\frac{\gamma}{\lambda_1}\left(\lambda_1\Delta_1 + 1\right)e^{-\lambda_1 \Delta_1} 
+
\frac{1-\gamma} {\lambda_2}\left(\lambda_2\Delta_2 + 1\right)e^{-\lambda_2 \Delta_2}
\right) (\gamma\lambda_1)e^{-\lambda_1\Delta_1}
\end{eqnarray*}
where
$$
\tau =
\frac{\frac{\gamma}{\lambda_1}\left(\lambda_1\Delta_1 + 1\right)e^{-\lambda_1 \Delta_1} 
+
\frac{1-\gamma} {\lambda_2}\left(\lambda_2\Delta_2 + 1\right)e^{-\lambda_2 \Delta_2}
}{(\gamma e^{-\lambda_1\Delta_1}+
(1-\gamma) e^{-\lambda_2\Delta_2})^2}
\neq 0
$$
Maxima implies
\begin{eqnarray*}
\gamma\lambda_1\left(\frac{\gamma}{\lambda_1}\left(\lambda_1\Delta_1 + 1\right)e^{-\lambda_1 \Delta_1} 
+
\frac{1-\gamma} {\lambda_2}\left(\lambda_2\Delta_2 + 1\right)e^{-\lambda_2 \Delta_2}
\right) e^{-\lambda_1\Delta_1}
&=& 
2\gamma\lambda_1\Delta_1\left(\gamma e^{-\lambda_1\Delta_1}+
(1-\gamma) e^{-\lambda_2\Delta_2}\right)
e^{-\lambda_1\Delta_1}
\\
\frac{\gamma}{\lambda_1}\left(\lambda_1\Delta_1 + 1\right)e^{-\lambda_1 \Delta_1} 
+
\frac{1-\gamma} {\lambda_2}\left(\lambda_2\Delta_2 + 1\right)e^{-\lambda_2 \Delta_2}
&=&
2\Delta_1\left(\gamma e^{-\lambda_1\Delta_1}+
(1-\gamma) e^{-\lambda_2\Delta_2}\right)
\end{eqnarray*}
For $\gamma=1$,
$\lambda_1\Delta_1=1$, reproducing the base case.
\\
Similarly,
\begin{eqnarray*}
&& \frac{1}{n}\cdot \frac{\partial}{\partial\Delta_2}E(\alpha^*,\Delta_1,\Delta_2) = 0
\\
&\Rightarrow & 
\frac{\gamma}{\lambda_1}\left(\lambda_1\Delta_1 + 1\right)e^{-\lambda_1 \Delta_1} 
+
\frac{1-\gamma} {\lambda_2}\left(\lambda_2\Delta_2 + 1\right)e^{-\lambda_2 \Delta_2}
=
2\Delta_2\left(\gamma e^{-\lambda_1\Delta_1}+
(1-\gamma) e^{-\lambda_2\Delta_2}\right)
\end{eqnarray*}
Let, 
$$
\lambda_1=k\cdot \lambda_2
$$
Let $\gamma=0.5, \lambda_1=1, \lambda_2=5$
\begin{eqnarray*}
\left(\Delta_1 + 1\right)e^{- \Delta_1} 
+
\frac{1} {5}\left(5\Delta_2 + 1\right)e^{-5 \Delta_2}
&=&
2\Delta_1\left(e^{-\Delta_1}+
e^{-5\Delta_2}\right)
\\
5\Delta_1e^{- \Delta_1} + 5e^{- \Delta_1} 
+
\left(5\Delta_2 + 1\right)e^{-5 \Delta_2}
&=&
10\Delta_1e^{-\Delta_1}+
10\Delta_1e^{-5\Delta_2}
\\
5e^{- \Delta_1} 
+
\left(5\Delta_2 + 1\right)e^{-5 \Delta_2}
&=&
5\Delta_1e^{-\Delta_1}+
10\Delta_1e^{-5\Delta_2}
\end{eqnarray*}
We assume $\sabs{\matW_i}\in [0,1]$, i.e., $0<c_1\Delta_1, c_2\Delta_2 <1$.
\fi
%========= begin remove ==============
\iffalse
\section{2-bit Ternary Weights}

Going below 4-bits we use the the ternary representation for weights, following the threshold based approximation proposed by Li et al [cite{}]. However, the main difference  is that instead of using only one scaling factor for a given layer, we use a separate scaling factor for each group of filters. This scheme seems to  be more appropriate for ternary approximation without using re-training to achieve better accuracy. Note that multiple scaling factors can lead to more high-precision compute. Therefore, we cluster filters carefully to improve the  ratio of low-precision to high-precision operations.
%$ \alpha^*, \hat\matW{}^* = \argmin_{\alpha,\hat\matW}\FsNorm{\matW-\alpha\hat\matW}^2\\
%&& s.t. \quad \alpha \ge 0, \hat\matW_i\in \{-1,0,+1\}, i=1,2,...,n
%\end{eqnarray*}
%
We mention the steps of our algorithms below. Ternarize-WithOut-Retraining (TwoR) takes the full-precision learned weights and returns the ternary representation of groups of filters along with their scaling factors. 
\\
\\
\textbf{Algorithm: Ternarize-WithOut-Retraining (TwoR)}\\
\\
\textbf{Input}: Learned weights \{\matW\} of a layer.
\\
\textbf{Steps}:\\
%For each layer:\\
1. Group $d$ filters into $k$ clusters: $\{G_j\}, j=1,..., k$. 
Let $s_j$ denote number of filters in cluster $G_j$.
\\
2. For each cluster $G_j$, 
\\
3. \quad Run \textbf{Alg:Threshold($\matW$)} on each filter $\matW \in G_j$, and store the thresholds as a vector $\alpha$.% (length $s_j$). 
%to return cluster of ternary filters $\hat G_j$ and corresponding scaling factor $\alpha_j$.
\\
4. \quad For $t=1,..., s_j$, \quad 
$T_t=\{i: \alpha_i \text{ belongs to the top } t \text{ elements from } \alpha\}$.
\\
%3. Construct $\hat\matW$, such that, $\hat\matW_i = Sign(\matW_i)$, for $i \in I$, and 0 otherwise. \\
5. \qquad Set $\alpha_t  = \sqrt{\sum_{i\in T_t}\alpha_i^2}$. 
\\
5. \qquad Construct $\hat\matW{}^{(t)}$, such that, $\hat\matW{}^{(t)}_i = Sign(\matW_i)$, if $\sabs{\matW_i} > \alpha_t$, and 0 otherwise. \\
%Use this as both threshold and scaling factor.
%\\
6. \quad Find $\alpha_{t^*}$ and $\hat\matW{}^*{}^{(t)}$ 
that minimizes 
$\sum_{\matW\in G_j}\FsNorm{\matW-\alpha_t\hat\matW{}^{(t)}}^2$.%/\FsNorm{\matW}^2$.
\\
7. Return $k$ number of $\alpha_{t^*}$ and the group of ternary weights $\hat\matW$.
\\
\\
\\
\textbf{Alg:Threshold (\matW)} :
\\
1. Sort weights $\matW$ ($n$ real numbers) according to magnitude.\\
%2. Let $\tau \in [0,1]$.\\
2. For $\tau \in [0,1]$, $I_\tau=\{i: \sabs{\matW_i} \text{ belongs to the top } \floor{\tau\cdot n} \text{ elements of sorted list}\}$.\\
%$\tilde \matW$ contains top $s = \floor{\tau\cdot n}$ elements (with sign) from sorted list. \\
3. Construct $\hat\matW{}^{(\tau)}$, such that, $\hat\matW{}^{(\tau)}_i = Sign(\matW_i)$, for $i \in I_\tau$, and 0 otherwise. \\
%5. Set scaling factor $\alpha_\tau=rms(\tilde\matW) = \sqrt{\sum_i \tilde\matW_i {}^2}$.\\
4. Set scaling factor $\alpha_\tau = \sqrt{\sum_{i\in I_\tau} \matW_i ^2}$.\\
5. Return $\alpha_{\tau^*}$ %and $\hat\matW$ 
that minimizes 
$\FsNorm{\matW-\alpha_\tau\hat\matW{}^{(\tau)}}^2$.%/\FsNorm{\matW}^2$.
\\
\\
We further quantize the scaling factors down to 8-bit to eliminate any operation that requires more than 8 bits. Applying this scheme on pre-trained ResNet-101 model, using 8-bit activations we achieve 71.8\% Top-1 accuracy on ImageNet dataset.
\fi
% =========== end remove ================
%\fi % === end of remove ===

==> new_formulation_main_old.tex <==
%================
\section{New Formulation}
%================
Let $\matM \in \mathbb{R}^{d\times r \times c}$ denote the full precision learned weight tensor for a given layer, where $d$ is the number of convolution filters and each filter is of dimension $r \times c$. We can unroll $\matM$ into a matrix $\matW \in \mathbb{R}^{d \times r\cdot c}$, where each row contains vector representation of a  convolution filter. We intend to find a ternary representation of $\matW$, denoted by $\hat\matW$, such that each element $\hat\matW_i \in \{-1,0,+1\}$. Current literature (reference 5) suggests to solve the following optimization problem in (\ref{eqn:current}).
%
\begin{eqnarray}\label{eqn:current}
\alpha^*, \hat\matW{}^* &=& \argmin_{\alpha,\hat\matW}\FsNorm{\matW-\alpha\hat\matW}^2\\
\nonumber 
&& s.t. \quad \alpha \ge 0, \hat\matW_i\in \{-1,0,+1\}, i=1,2,...,n
\end{eqnarray}
Note that here we approximate the ternary representation using only one scaling factor $\alpha$. However, we found this formulation to be ineffective for conversion of full-precision trained weights to low-precision, when we do not use re-training. Instead, we seek to find an $\alpha$ for each filter (or a cluster of filters) for better accuracy. Specifically, we intend to solve ()


\subsection{Element-wise $\alpha$}
\begin{eqnarray*}
\matA^*, \hat\matW{}^* &=& \argmin_{\matA,\hat\matW}\FsNorm{\matW-\matA\odot\hat\matW}^2\\
&& s.t. \quad \matA_i \ge 0, \hat\matW_i\in \{-1,0,+1\}, i=1,2,...,n
\end{eqnarray*}

\subsection{Filter-wise $\alpha$}
\begin{eqnarray*}
a_j^*, \hat\matW{}^* &=& \argmin_{a_j,\hat\matW}\sum_j\FsNorm{\matW^{(j)}-a_j\hat\matW{}^{(j)}}^2\\
&& s.t. \quad a_j \ge 0, \hat\matW_i{}^{(j)}\in \{-1,0,+1\}, i=1,2,...,n; j=1,...,d
\end{eqnarray*}
Equivalently, for a diagonal matrix $\matD \ge 0$,
\begin{eqnarray*}
\matD^*, \hat\matW{}^* &=& \argmin_{\matD,\hat\matW}\FsNorm{\matW-\matD\hat\matW}^2\\
&& s.t. \quad \matD_i \ge 0, \hat\matW_i\in \{-1,0,+1\}, i=1,2,...,n;
\end{eqnarray*}
Equivalently, for a diagonal matrix $\matD \ge 0$,
\begin{eqnarray*}
\matW &=& Sign(\matW)\odot\sabs{\matW}
\\
\matD\hat\matW &=& \matD (Sign(\matW)\odot \tilde\matW) 
=  Sign(\matW)\odot (\matD\tilde\matW)
\end{eqnarray*}
\begin{eqnarray*}
\FsNorm{\matW - \matD\hat\matW}^2 &=& \FsNorm{Sign(\matW)\odot\sabs{\matW}
- Sign(\matW)\odot (\matD\tilde\matW)}^2
%\matD\hat\matW &=& \matD (Sign(\matW)\odot \tilde\matW) 
%=  Sign(\matW)\odot (\matD\tilde\matW)
\\
&=& \FsNorm{\sabs{\matW}
- \matD\tilde\matW}^2
\end{eqnarray*}
\begin{eqnarray*}
%\matD^*, \tilde\matW{}^* &=& \argmin_{\matD,\tilde\matW}\frac{\FsNorm{\sabs{\matW}-\matD\tilde\matW}^2}{\FsNorm{\matW}^2}\\
\matD^*, \tilde\matW{}^* &=& \argmin_{\matD,\tilde\matW}\FsNorm{\sabs{\matW}-\matD\tilde\matW}^2\\&& s.t. \quad \matD_i \ge 0, \tilde\matW_i\in \{0, 1\}, i=1,2,...,n;
\\
\hat\matW &=& Sign(\matW)\odot \tilde\matW
\end{eqnarray*}
Optimal $\matD_i^*$ can be computed as, for a given $\hat\w$ (depends on $\Delta^*$,
$$
\matD_i^* = \frac{\w^T\hat\w}{\FsNorm{\hat\w}^2}
$$
$$
\Delta^* = \argmax_{\Delta>0}\frac{1}{\sabs{I_\Delta}}(\sum_{i\in I_\Delta}\sabs{\matW_i})^2
$$
\subsection{Cluster-wise $\alpha$}

Let diagonal matrix $\tilde\matD$ denote the cluster of scaling factors, where scaling factors are assigned their cluster centroids. For $k$ clusters we have $k$ unique values of  $\tilde\matD$. Also, let $\hat\matD$ denote the low-precision representation of cluster centroids. Then, sub-8 decomposition looks like $\hat\matD\hat\matW$ and the following holds
\begin{eqnarray*}
\FsNorm{\matW-\hat\matD\hat\matW{}^*}
&\leq& 
\FsNorm{\matW-\tilde\matD\hat\matW{}^*}+\FsNorm{\tilde\matD\hat\matW-\hat\matD\hat\matW{}^*}\\
&\leq&
\FsNorm{\matW-\matD{}^*\hat\matW{}^*}+\FsNorm{\matD{}^*\hat\matW{}^*-\tilde\matD\hat\matW{}^*}+\FsNorm{\tilde\matD\hat\matW{}^*-\hat\matD\hat\matW{}^*}\\
&\leq&
\underbrace{\FsNorm{\matW-\matD{}^*\hat\matW{}^*}}_{\text{Ternarization error}}+\underbrace{\FsNorm{\matD{}^*-\tilde\matD}\FsNorm{\hat\matW{}^*}}_{\text{Clustering error}}+\underbrace{\FsNorm{\tilde\matD-\hat\matD}\FsNorm{\hat\matW{}^*}}_{\text{Error for low-precision scaling factors}}\\
\end{eqnarray*}
Error bound due to clustering $\FsNorm{\matD-\tilde\matD}\FsNorm{\hat\matW}$ holds for any clustering (static or dynamic); however, static clustering may give us bigger error whereas optimal clustering $k$-means can make the error smaller. On the other hand, static clustering can give a performance boost while $k$-means may not.

\subsection{Layer-wise $\alpha$}
\begin{eqnarray*}
\alpha^*, \hat\matW{}^* &=& \argmin_{\alpha,\hat\matW}\FsNorm{\matW-\alpha\hat\matW}^2\\
&& s.t. \quad \alpha \ge 0, \hat\matW_i\in \{-1,0,+1\}, i=1,2,...,n
\end{eqnarray*}

%\section{Algorithm: Ternarize-WithOut-Retraining (TwoR)}


%\input{algo_LP}
\subsection{General Bound/Analysis}
$$
E(\hat\w,\alpha) = \FsNorm{\w - \alpha\hat\w}^2
= \FsNorm{\w}^2 - 2\alpha \w^T\hat\w + \alpha^2\FsNorm{\hat\w}^2
$$
Given $\hat\w$, optimal $\alpha^*$ is
$$
\alpha^* = \frac{\w^T\hat\w}{\FsNorm{\hat\w}^2}
$$
$$
E(\hat\w,\alpha^*) 
= \FsNorm{\w}^2 - 2\frac{(\w^T\hat\w)^2}{\FsNorm{\hat\w}^2} + \frac{(\w^T\hat\w)^2}{\FsNorm{\hat\w}^2}
= \FsNorm{\w}^2 - \frac{(\w^T\hat\w)^2}{\FsNorm{\hat\w}^2}
$$
So, minimizing $E$ is maximizing $\frac{(\w^T\hat\w)^2}{\FsNorm{\hat\w}^2}$.
\subsubsection{Ternary Weights}
For ternary representation (keeping weights above some threshold along with their sign)
$$
\w^T\hat\w = \sum_{i\in I_\Delta} \sabs{\w_i}
$$
and
$$
\FsNorm{\hat\w}^2 = \sabs{I_\Delta}
$$

\subsubsection{Binary Weights}
$$
\FsNorm{\hat\w}^2 = n
$$
We want to maximize $\sabs{\w^T\hat\w}$.

\subsection{Quantization using Data}
\begin{eqnarray*}
\matD^*, \hat\matW{}^* &=& \argmin_{\matD,\hat\matW}\sum_{\x\in\mathcal{X}}\FsNorm{\matW\x-\matD\hat\matW\x}^2\\
&& s.t. \quad \matD_i \ge 0, \hat\matW_i\in \{-1,0,+1\}, i=1,2,...,n;
%\end{eqnarray*}
%\begin{eqnarray*}
\\
\alpha_j^*, \hat\matW{}^{(j)}{}^* &=& \argmin_{\alpha_j,\hat\matW}\sum_{\x\in\mathcal{X}}\FsNorm{\matW^{(j)}\x-\alpha_j\hat\matW{}^{(j)}\x}^2\\
&& s.t. \quad \alpha_j \ge 0, \hat\matW_i{}^{(j)}\in \{-1,0,+1\}, i=1,2,...,n; j=1,...,d
\end{eqnarray*}

\section{Residual Precision}
$\matW$ full precision weight\\
$\hat\matW$ ternary weight with 8-bit scaling factor $\hat\alpha$\\
$\Delta = \matW - \hat\alpha\hat\matW$ full precision residual\\
$\hat\Delta$ is ternary residual precision with 8-bit scaling factor $\hat\delta$ 
$$
e = \FsNorm{\matW - (\hat\alpha\hat\matW+\hat\delta\hat\Delta)}
= \FsNorm{\Delta-\hat\delta\hat\Delta}
\geq 
\FsNorm{\Delta}-\FsNorm{\hat\delta\hat\Delta}
$$
$$
\FsNorm{\Delta}-e \leq \FsNorm{\hat\delta\hat\Delta}
$$
Error reduction can be up to $\FsNorm{\hat\delta\hat\Delta}$.

\section{TWN proof}
We want to solve the following
$$
\Delta^* = \argmax_{\Delta>0} \quad \frac{1}{\sabs{I_\Delta}}(\sum_{i\in I_\Delta} \sabs{\matW_i})^2 
$$
\subsection{Uniform case}
Let $\x \sim \mathcal{U}[-a,+a]$. 
%Then, $\mathbb{E}(\sabs{\x}) = \frac{1}{3}a$ as follows.
\begin{eqnarray*}
I(t) = \frac{1}{a}\int_{t}^{a} x dx
= \frac{a^2-t^2}{2a} 
= \frac{(a+t)(a-t)}{2a}
\end{eqnarray*}
$$
\Delta^* = \argmax_t F(t) = \argmax_t \frac{1}{4a^2}\frac{(a+t)^2(a-t)^2}{a-t}
 = \argmax_t \frac{1}{4a^2}(a+t)^2(a-t)
$$
$$
f'(t) = 0 \Rightarrow \Delta^* = a/3
$$
`\subsection{Gaussian case}
Let $\x \sim \mathcal{N}(0,\sigma^2)$. Then, $\mathbb{E}(\sabs{\x}) = 0.8\sigma$ as follows.
\begin{eqnarray*}
I = \frac{1}{\sigma\sqrt{2\pi}}\int_{-\infty}^{\infty}e^{-\frac{\sabs{x}^2}{2\sigma^2}}\sabs{x}dx
= \frac{\sqrt{2}}{\sigma\sqrt{\pi}}\int_{0}^{\infty}e^{-\frac{x^2}{2\sigma^2}}x dx
\end{eqnarray*}
Let $y=\frac{x^2}{2\sigma^2}$, then, $x dx = \sigma^2 dy$
\begin{eqnarray*}
I = {\sigma}\frac{\sqrt{2}}{\sqrt{\pi}}\int_{0}^{\infty} e^{-y}dy
= - {\sigma}\frac{\sqrt{2}}{\sqrt{\pi}} e^{-y}\Big]_0^\infty
= {\sigma}\frac{\sqrt{2}}{\sqrt{\pi}}
\approx 0.8\sigma
\end{eqnarray*}

We want to keep top elements that maximize ratio of the above integral and square root of number of elements we keep.
$$
F(t) = \frac{\sqrt{2}}{\sigma\sqrt{\pi}}\int_{t}^{a}\frac{e^{-\frac{x^2}{2\sigma^2}}x}{\sqrt{a-t}} dx
$$
$$
\argmax_t \quad F(t)
$$
\subsection{Exponential Case}
$$
%\sabs{I_\Delta} = n \int_{x>\Delta} f(x)dx  
\sabs{I_\Delta} \approx n \int_{x>\Delta} f(x)dx 
= n \left(1 - \int_{x <= \Delta} f(x)dx\right)
= n(1-F(\Delta))
$$
where $f(x)=\lambda e^{-\lambda x}$ is pdf of exponential distribution with parameter $\lambda>0$, and $F(x) = 1-e^{-\lambda x}$ is the cdf.
Therefore, 
$$
\sabs{I_\Delta} \approx n e^{-\lambda\Delta}
$$
Furthermore,
$$
\sum_{i\in I_\Delta}\sabs{W_i} \approx n \int_{x>\Delta} x f(x)dx
= n \int_{x>\Delta} (\lambda e^{-\lambda x})x dx
$$
Using integration by parts
$$
\sum_{i\in I_\Delta}\sabs{W_i} \approx n \left(-xe^{-\lambda x}\Big]_{x>\Delta}- \int_{x>\Delta} (-e^{-\lambda x})dx\right)
= n \left(-xe^{-\lambda x}\Big]_{x>\Delta}- \frac{1}{\lambda} e^{-\lambda x}\Big]_{x>\Delta}\right)
$$
From L'hospital's rule
$$
L = \lim_{x \rightarrow \infty}\frac{x}{e^{\lambda x}}
= \lim_{x \rightarrow \infty}\frac{\lambda}{e^{\lambda x}}
= 0
$$
Therefore,
$$
\sum_{i\in I_\Delta}\sabs{W_i} \approx n\left(\Delta e^{-\lambda \Delta}+\frac{1}{\lambda}e^{-\lambda \Delta}\right)
$$
Then,
$$
G(\Delta) = \frac{(\sum_{i\in I\Delta}\sabs{W_i})^2}{\sabs{I_\Delta}}
= \frac{1}{\lambda^2}(1+\lambda\Delta)^2e^{-\lambda\Delta}
$$
$$
G'(\Delta) = \frac{1}{\lambda^2}(2\lambda(1+\lambda\Delta)e^{-\lambda\Delta}-\lambda(1+\lambda\Delta)^2e^{-\lambda\Delta})
$$
$$
G'(\Delta) = 0 \Rightarrow \Delta = \frac{1}{\lambda}
$$
$$
G''(\Delta)\Big|_{\Delta=1/\lambda} < 0 \quad \text{(maxima)}
$$
Therefore,
$$
\Delta^* = \frac{1}{\lambda} = \frac{1}{n}\sum_i\sabs{\matW_i}
$$
\section{Improved Formulation}
\subsection{Two thresholds, two $\alpha$}
Positive and negative values may not be distributed identically. We use separate thresholds and scaling factors for positive and negative weights, and compute respective optima.
\begin{eqnarray*}
I_+ &=& \{i: W_i > \Delta_+\}
\\
I_- &=& \{i: W_i < -\Delta_-\}
\end{eqnarray*}
\begin{eqnarray*}
\Delta_+^* &=& \argmax_{\Delta_+>0} \quad \frac{1}{\sabs{I_+}}(\sum_{i\in I_+} \sabs{\matW_i})^2 
\\
\alpha_+^* &=& \frac{1}{\sabs{I_+}}\sum_{i\in I_+} \sabs{\matW_i}
\\
\Delta_-^* &=& \argmax_{\Delta_->0} \quad \frac{1}{\sabs{I_-}}(\sum_{i\in I_+} \sabs{\matW_i})^2 
\\
\alpha_-^* &=& \frac{1}{\sabs{I_-}}\sum_{i\in I_-} \sabs{\matW_i}
\end{eqnarray*}
We can split $\matW$ into positive and negative components 
$$
\matW = \matW_+ + \matW_-.
$$
Let the corresponding optimal ternary representations be $\alpha_+^*\hat\matW_+^*$ and $\alpha_-^*\hat\matW_-^*$.
\\
The ternarization error is
\begin{eqnarray*}
E &=& \FsNorm{\matW - (\alpha_+^*\hat\matW_+^* + \alpha_-^*\hat\matW_-^* )}^2\\
%\Delta_+^* &=& \argmax_{\Delta_+>0} \quad \frac{1}{\sabs{I_+}}(\sum_{i\in I_+} \sabs{\matW_i})^2 
%\\
%\alpha_+^* &=& \frac{1}{\sabs{I_+}}\sum_{i\in I_+} \sabs{\matW_i}
\end{eqnarray*}

\section{Additional Experiments}

1. Layer-wise $\alpha$: Gaussian TWN vs Exponential vs positive-negative $\alpha$.\\
- plot all the errors
\\
\\
2. Hierarchical vs non-hierarchical\\
- cluster the filters and find one $\alpha$ and $\Delta$ for the entire cluster (without hierarchical )
\\
- 
\section{Bound for Hierarchical}
Split $\w$ into two orthogonal components
$$
\w = \w_p + \w_n
$$
Optimal ternary for $\w_p$ and $\w_n$ are given as $\alpha_p^*\hat\w_p^*$ and $\alpha_n^*\hat\w_n^*$, respectively. 
\begin{eqnarray*}
\epsilon^* 
&=& \FsNorm{\w - \alpha_p^*\hat\w_p^* - \alpha_n^*\hat\w_n^*}^2
= \FsNorm{\w_p - \alpha_p^*\hat\w_p^*}^2 + \FsNorm{\w_n - \alpha_n^*\hat\w_n^*}^2
\end{eqnarray*}
%
\begin{eqnarray*}
\epsilon
&=& \FsNorm{\w - \alpha_p^*\hat\w_p^* - \alpha_n^*\hat\w_n^*}^2
= \FsNorm{\w_p - \alpha_p^*\hat\w_p^*}^2 + \FsNorm{\w_n - \alpha_n^*\hat\w_n^*}^2
\end{eqnarray*}

\section{Mixture Distribution}
Use one $\alpha$ but two thersholds: for positive and negative numbers.
\\
\begin{eqnarray*}
\hat\matW_i &=& 1, \quad if \quad \matW_i > \Delta_p,
\\
\hat\matW_i &=& -1, \quad if \quad \matW_i < -\Delta_n,
\end{eqnarray*}
Let 
$$
I_\Delta^+ = \{i: \matW_i > \Delta_p\}
$$
$$
I_\Delta^- = \{i: \matW_i < -\Delta_n\}
$$
We want to solve
$$
\alpha^*,\Delta_p^*,\Delta_n^*
= \argmin_{\alpha\geq 0,\Delta_p>0,\Delta_n>0}
\FsNorm{\matW - \alpha\hat\matW}^2
$$
\begin{eqnarray*}
E(\alpha,\Delta_p,\Delta_n) &=& \FsNorm{\matW - \alpha\hat\matW}^2
\\
&=&
\sum_i \matW_i^2 - 2\alpha\sum_i\matW_i\hat\matW_i + \alpha^2\sum_i \hat\matW_i{}^2
\\
&=& \sum_i \matW_i^2 - 2\alpha(\sum_{i\in I_\Delta^+}\matW_i\hat\matW_i+\sum_{i\in I_\Delta^-}\matW_i\hat\matW_i) + \alpha^2(\sum_{i\in I_\Delta^+}\hat\matW_i{}^2 + \sum_{i\in I_\Delta^-}\hat\matW_i{}^2)
\end{eqnarray*}
We have
$$
\sum_{i\in I_\Delta^+}\hat\matW_i{}^2
= \sabs{I_\Delta^+},
\quad 
\sum_{i\in I_\Delta^-}\hat\matW_i{}^2
= \sabs{I_\Delta^-}
$$
$$
\sum_{i\in I_\Delta^+}\matW_i\hat\matW_i{}
= \sum_{i\in I_\Delta^+}\sabs{\matW_i},
\quad
\sum_{i\in I_\Delta^-}\matW_i\hat\matW_i{}
= \sum_{i\in I_\Delta^-}\sabs{\matW_i}
$$
$$
\frac{\partial}{\partial\alpha} E(\alpha,\Delta_p,\Delta_n)
= 2\alpha(\sabs{I_\Delta^+} + \sabs{I_\Delta^-}) - 2(\sum_{i\in I_\Delta^+}\sabs{\matW_i}+\sum_{i\in I_\Delta^-}\sabs{\matW_i})
$$
For fixed $\Delta_p$, $\Delta_n$, $E$ attains maxima at 
$$
\alpha^* = \frac{\sum_{i\in I_\Delta^+}\sabs{\matW_i}+\sum_{i\in I_\Delta^-}\sabs{\matW_i}}{\sabs{I_\Delta^+} + \sabs{I_\Delta^-}}
$$
Using this optimal expression we have 
\begin{eqnarray*}
E(\alpha^*,\Delta_p,\Delta_n)
&=& \sum_i\matW_i^2 - \frac{(\sum_{i\in I_\Delta^+}\sabs{\matW_i}+\sum_{i\in I_\Delta^-}\sabs{\matW_i})^2}{\sabs{I_\Delta^+} + \sabs{I_\Delta^-}}
\end{eqnarray*}
\begin{eqnarray*}
\Delta_p^*,\Delta_n^* &=& \argmax_{\Delta_p,\Delta_n} \frac{(\sum_{i\in I_\Delta^+}\sabs{\matW_i}+\sum_{i\in I_\Delta^-}\sabs{\matW_i})^2}{\sabs{I_\Delta^+} + \sabs{I_\Delta^-}}
\end{eqnarray*}
We assume that positive weights follow exponential distribution with parameter $\lambda_1$, and magnitude of negative weights follow exponential distribution with parameter $\lambda_2$.
\\
Let $\gamma\in [0,1]$ be a mixing parameter, i.e., $\gamma n$ number of positive elements and $(1-\gamma)n$ number of negative elements.
$$
\sabs{I_\Delta^+} \approx \gamma n e^{-\lambda_1\Delta_1},
\quad 
\sabs{I_\Delta^-} \approx (1-\gamma) n e^{-\lambda_2\Delta_2}
$$
Furthermore,
$$
\sum_{i\in I_\Delta^+}\sabs{W_i} \approx \frac{\gamma n}{\lambda_1}\left(\lambda_1\Delta_1 + 1\right)e^{-\lambda_1 \Delta_1}
$$
$$
\sum_{i\in I_\Delta^-}\sabs{W_i} \approx \frac{(1-\gamma) n}{\lambda_2}\left(\lambda_2\Delta_2 + 1\right)e^{-\lambda_2 \Delta_2}
$$
\begin{eqnarray*}
E(\alpha^*,\Delta_1,\Delta_2)
&=& 
n\frac{\left(\frac{\gamma}{\lambda_1}\left(\lambda_1\Delta_1 + 1\right)e^{-\lambda_1 \Delta_1} 
+
\frac{1-\gamma} {\lambda_2}\left(\lambda_2\Delta_2 + 1\right)e^{-\lambda_2 \Delta_2}
\right)^2}{\gamma e^{-\lambda_1\Delta_1}+
(1-\gamma) e^{-\lambda_2\Delta_2}}
\end{eqnarray*}
It follows
\begin{eqnarray*}
&&\frac{1}{n}\cdot \frac{\partial}{\partial\Delta_1}E(\alpha^*,\Delta_1,\Delta_2)\\
&=& 
\frac{2\left(\frac{\gamma}{\lambda_1}\left(\lambda_1\Delta_1 + 1\right)e^{-\lambda_1 \Delta_1} 
+
\frac{1-\gamma} {\lambda_2}\left(\lambda_2\Delta_2 + 1\right)e^{-\lambda_2 \Delta_2}
\right)\left[\frac{\gamma}{\lambda_1}(\lambda_1e^{-\lambda_1 \Delta_1}-(\lambda_1\Delta_1+1)\lambda_1e^{-\lambda_1 \Delta_1})\right]}{\gamma e^{-\lambda_1\Delta_1}+
(1-\gamma) e^{-\lambda_2\Delta_2}}
\\
&& -
\frac{\left(\frac{\gamma}{\lambda_1}\left(\lambda_1\Delta_1 + 1\right)e^{-\lambda_1 \Delta_1} 
+
\frac{1-\gamma} {\lambda_2}\left(\lambda_2\Delta_2 + 1\right)e^{-\lambda_2 \Delta_2}
\right)^2}{(\gamma e^{-\lambda_1\Delta_1}+
(1-\gamma) e^{-\lambda_2\Delta_2})^2}\gamma (-\lambda_1) e^{-\lambda_1\Delta_1}
\\
&=&\tau \cdot 
2\left(\gamma e^{-\lambda_1\Delta_1}+
(1-\gamma) e^{-\lambda_2\Delta_2}\right)
\left[\gamma(-\lambda_1\Delta_1)e^{-\lambda_1\Delta_1}\right]
+
\\
&&
\tau \cdot 
\left(\frac{\gamma}{\lambda_1}\left(\lambda_1\Delta_1 + 1\right)e^{-\lambda_1 \Delta_1} 
+
\frac{1-\gamma} {\lambda_2}\left(\lambda_2\Delta_2 + 1\right)e^{-\lambda_2 \Delta_2}
\right) (\gamma\lambda_1)e^{-\lambda_1\Delta_1}
\end{eqnarray*}
where
$$
\tau =
\frac{\frac{\gamma}{\lambda_1}\left(\lambda_1\Delta_1 + 1\right)e^{-\lambda_1 \Delta_1} 
+
\frac{1-\gamma} {\lambda_2}\left(\lambda_2\Delta_2 + 1\right)e^{-\lambda_2 \Delta_2}
}{(\gamma e^{-\lambda_1\Delta_1}+
(1-\gamma) e^{-\lambda_2\Delta_2})^2}
\neq 0
$$
Maxima implies
\begin{eqnarray*}
\gamma\lambda_1\left(\frac{\gamma}{\lambda_1}\left(\lambda_1\Delta_1 + 1\right)e^{-\lambda_1 \Delta_1} 
+
\frac{1-\gamma} {\lambda_2}\left(\lambda_2\Delta_2 + 1\right)e^{-\lambda_2 \Delta_2}
\right) e^{-\lambda_1\Delta_1}
&=& 
2\gamma\lambda_1\Delta_1\left(\gamma e^{-\lambda_1\Delta_1}+
(1-\gamma) e^{-\lambda_2\Delta_2}\right)
e^{-\lambda_1\Delta_1}
\\
\frac{\gamma}{\lambda_1}\left(\lambda_1\Delta_1 + 1\right)e^{-\lambda_1 \Delta_1} 
+
\frac{1-\gamma} {\lambda_2}\left(\lambda_2\Delta_2 + 1\right)e^{-\lambda_2 \Delta_2}
&=&
2\Delta_1\left(\gamma e^{-\lambda_1\Delta_1}+
(1-\gamma) e^{-\lambda_2\Delta_2}\right)
\end{eqnarray*}
For $\gamma=1$,
$\lambda_1\Delta_1=1$, reproducing the base case.
\\
Similarly,
\begin{eqnarray*}
&& \frac{1}{n}\cdot \frac{\partial}{\partial\Delta_2}E(\alpha^*,\Delta_1,\Delta_2) = 0
\\
&\Rightarrow & 
\frac{\gamma}{\lambda_1}\left(\lambda_1\Delta_1 + 1\right)e^{-\lambda_1 \Delta_1} 
+
\frac{1-\gamma} {\lambda_2}\left(\lambda_2\Delta_2 + 1\right)e^{-\lambda_2 \Delta_2}
=
2\Delta_2\left(\gamma e^{-\lambda_1\Delta_1}+
(1-\gamma) e^{-\lambda_2\Delta_2}\right)
\end{eqnarray*}
Let, 
$$
\lambda_1=k\cdot \lambda_2
$$
Let $\gamma=0.5, \lambda_1=1, \lambda_2=5$
\begin{eqnarray*}
\left(\Delta_1 + 1\right)e^{- \Delta_1} 
+
\frac{1} {5}\left(5\Delta_2 + 1\right)e^{-5 \Delta_2}
&=&
2\Delta_1\left(e^{-\Delta_1}+
e^{-5\Delta_2}\right)
\\
5\Delta_1e^{- \Delta_1} + 5e^{- \Delta_1} 
+
\left(5\Delta_2 + 1\right)e^{-5 \Delta_2}
&=&
10\Delta_1e^{-\Delta_1}+
10\Delta_1e^{-5\Delta_2}
\\
5e^{- \Delta_1} 
+
\left(5\Delta_2 + 1\right)e^{-5 \Delta_2}
&=&
5\Delta_1e^{-\Delta_1}+
10\Delta_1e^{-5\Delta_2}
\end{eqnarray*}
We assume $\sabs{\matW_i}\in [0,1]$, i.e., $0<c_1\Delta_1, c_2\Delta_2 <1$.
%========= begin remove ==============
\iffalse
\section{2-bit Ternary Weights}

Going below 4-bits we use the the ternary representation for weights, following the threshold based approximation proposed by Li et al [cite{}]. However, the main difference  is that instead of using only one scaling factor for a given layer, we use a separate scaling factor for each group of filters. This scheme seems to  be more appropriate for ternary approximation without using re-training to achieve better accuracy. Note that multiple scaling factors can lead to more high-precision compute. Therefore, we cluster filters carefully to improve the  ratio of low-precision to high-precision operations.
%$ \alpha^*, \hat\matW{}^* = \argmin_{\alpha,\hat\matW}\FsNorm{\matW-\alpha\hat\matW}^2\\
%&& s.t. \quad \alpha \ge 0, \hat\matW_i\in \{-1,0,+1\}, i=1,2,...,n
%\end{eqnarray*}
%
We mention the steps of our algorithms below. Ternarize-WithOut-Retraining (TwoR) takes the full-precision learned weights and returns the ternary representation of groups of filters along with their scaling factors. 
\\
\\
\textbf{Algorithm: Ternarize-WithOut-Retraining (TwoR)}\\
\\
\textbf{Input}: Learned weights \{\matW\} of a layer.
\\
\textbf{Steps}:\\
%For each layer:\\
1. Group $d$ filters into $k$ clusters: $\{G_j\}, j=1,..., k$. 
Let $s_j$ denote number of filters in cluster $G_j$.
\\
2. For each cluster $G_j$, 
\\
3. \quad Run \textbf{Alg:Threshold($\matW$)} on each filter $\matW \in G_j$, and store the thresholds as a vector $\alpha$.% (length $s_j$). 
%to return cluster of ternary filters $\hat G_j$ and corresponding scaling factor $\alpha_j$.
\\
4. \quad For $t=1,..., s_j$, \quad 
$T_t=\{i: \alpha_i \text{ belongs to the top } t \text{ elements from } \alpha\}$.
\\
%3. Construct $\hat\matW$, such that, $\hat\matW_i = Sign(\matW_i)$, for $i \in I$, and 0 otherwise. \\
5. \qquad Set $\alpha_t  = \sqrt{\sum_{i\in T_t}\alpha_i^2}$. 
\\
5. \qquad Construct $\hat\matW{}^{(t)}$, such that, $\hat\matW{}^{(t)}_i = Sign(\matW_i)$, if $\sabs{\matW_i} > \alpha_t$, and 0 otherwise. \\
%Use this as both threshold and scaling factor.
%\\
6. \quad Find $\alpha_{t^*}$ and $\hat\matW{}^*{}^{(t)}$ 
that minimizes 
$\sum_{\matW\in G_j}\FsNorm{\matW-\alpha_t\hat\matW{}^{(t)}}^2$.%/\FsNorm{\matW}^2$.
\\
7. Return $k$ number of $\alpha_{t^*}$ and the group of ternary weights $\hat\matW$.
\\
\\
\\
\textbf{Alg:Threshold (\matW)} :
\\
1. Sort weights $\matW$ ($n$ real numbers) according to magnitude.\\
%2. Let $\tau \in [0,1]$.\\
2. For $\tau \in [0,1]$, $I_\tau=\{i: \sabs{\matW_i} \text{ belongs to the top } \floor{\tau\cdot n} \text{ elements of sorted list}\}$.\\
%$\tilde \matW$ contains top $s = \floor{\tau\cdot n}$ elements (with sign) from sorted list. \\
3. Construct $\hat\matW{}^{(\tau)}$, such that, $\hat\matW{}^{(\tau)}_i = Sign(\matW_i)$, for $i \in I_\tau$, and 0 otherwise. \\
%5. Set scaling factor $\alpha_\tau=rms(\tilde\matW) = \sqrt{\sum_i \tilde\matW_i {}^2}$.\\
4. Set scaling factor $\alpha_\tau = \sqrt{\sum_{i\in I_\tau} \matW_i ^2}$.\\
5. Return $\alpha_{\tau^*}$ %and $\hat\matW$ 
that minimizes 
$\FsNorm{\matW-\alpha_\tau\hat\matW{}^{(\tau)}}^2$.%/\FsNorm{\matW}^2$.
\\
\\
We further quantize the scaling factors down to 8-bit to eliminate any operation that requires more than 8 bits. Applying this scheme on pre-trained ResNet-101 model, using 8-bit activations we achieve 71.8\% Top-1 accuracy on ImageNet dataset.
\fi
% =========== end remove ================

==> training.tex <==
\section{Training with Low-precision}
{\label{sec_lptrain}}
We trained the low precision ResNet-50 on ImageNet dataset using 2-bit weights and 8-bit activations by initializing the network with pre-trained full precision model. We take the approach proposed by Marcel et al.\cite{marcelbatchnorm}, and replace data pre-processing steps such as mean-subtraction and jittering with batch normalization layer inserted right after the data later. We obtained the pre-trained models published by Marcel et al.\cite{marcelbatchnorm} and fine-tune the parameters of our low-precision network. In the forward pass, the weights are converted to 2-bit ternary values using the algorithm described in \ref{alg:TwoR} in all convolution layers, except the first layer, where the weights are quantized to 8-bit fixed point representation. Activations are quantized to 8-bit fixed point in all layers including ReLU, BatchNorm layers. We did not quantize the weights in FC layer for the training exercise. Gradient updates are performed in full precision for convolution and FC layers. We reduced the learning rate to an order of 1e-4, in order to avoid exploding gradients problem, while we keep all the other hyper parameters same as that of full precision training. After running for 4-epochs, we recovered most of the accuracy and achieved $68.6\%$ Top-1 and $88.7\%$ Top-5 accuracy compared to our baseline $75.02\%$(Top-1), $92.2\%$(Top-5). 

\begin{figure}[h]
\centering
\includegraphics[width=.9\columnwidth]{plots/resnet50_train_2.png}
\centering
\caption{Fine-tuning Resnet-50 with pre-initialized weights on Imagenet dataset.} \label{fig_res101}
\end{figure}

